NLTGCR: A class of Nonlinear Acceleration Procedures based on Conjugate Residuals

This paper develops a new class of nonlinear acceleration algorithms based on extending conjugate residual-type procedures from linear to nonlinear equations. The main algorithm has strong similarities with Anderson acceleration as well as with inexact Newton methods - depending on which variant is implemented. We prove theoretically and verify experimentally, on a variety of problems from simulation experiments to deep learning applications, that our method is a powerful accelerated iterative algorithm.

==> exper.tex <==
 
 \section{Numerical experiments}
This section compares nlTGCR to existing methods in the
literature through several numerical experiments. We first introduce an adaptive mechanism that combines the nonlinear update version and the linearized update version. Then we show features of nlTGCR, saying memory efficiency and fast convergence in the first several steps, with problems in both systems of nonlinear equations and optimization. In the end, we also discuss the cases where the gradients are stochastic.

All experiments were performed on a workstation with an Intel i7-9700k CPU and an NVIDIA GeForce RTX 2070 GPU. The first three experiments were implemented in Matlab 2022b, and the baseline methods were based on the implementation of H. Kasai~\cite{gdlibrary} and C.T. Kelley~\cite{kelley_solving_2003}. The GNN frameworks were based mainly on PyTorch~\cite{pytorch} and PyTorch-Geometric~\cite{pyg}.

\subsection{Bratu problem}
We consider a nonlinear PDE problem, namely the Bratu problem~\cite{hajipour2018accurate}, of the form:
      {\begin{align*}
         \Delta u + \lambda e^ u &= 0  \ \ \text{in} \ \ \Omega = (0, 1)\times (0,1)  \\
          u(x,y)  &= 0  \ \text{for} \  (x,y) \in \partial \Omega  
        \end{align*} 
In the following experiment we take $\lambda = 0.5$. The problem is discretized with Centered Finite Differences~\cite{chaudhry2008open,folland1995introduction,wilmott1995mathematics} using a grid of size $100 \times 100 $. This leads to a problem of solving a nonlinear equation $f(s) = 0$ with $s \in \mathbb{R}^{10000}$ and $f:\mathbb{R}^{10000}\to\mathbb{R}^{10000}$. The corresponding fixed point problem is $g(s) = s + \beta f(s)$.

\subsubsection{Adaptive update version}



\begin{figure}
      \parbox{0.48\textwidth}      {\includegraphics[width=0.48\textwidth]{Bratu_mode_feval.eps}
      \caption{Function evaluation - Cost of the Bratu problem. Each marker represents 20 iterations.\label{fig:bratu_mode_1}}}
      \hfill
      \parbox{0.48\textwidth}{\includegraphics[width=0.48\textwidth]{Bratu_mode_iter.eps}
      \caption{Iteration - Cost figure of the Bratu problem. Each marker represents 20 iterations. \label{fig:bratu_mode_2}}}
\end{figure}

A property of the Bratu problem is that it is almost linear despite the exponential term. This property also appears in many applications when getting close to convergence. Therefore, the linearized update version of nlTGCR is worth consideration since it can half the number of function evaluations if using complex differentiation. Nonetheless, without the help of carefully selected restarting, the linear update version is usually less robust than the nonlinear one in avoiding stagnation. Here, we introduce an adaptive mechanism that switches from the nonlinear update to the linear update when the problem is nearly linear and switches back when it needs to restart or clear the memory. Let $r^{nl}_j$ and $r^{lin}_j$ denote the nonlinear and linear residuals at iteration $j$ such that
\begin{equation}
    r^{nl}_{j+1} = -f(x_{j+1}), \ \ 
    r^{lin}_{j+1} = r^{nl}_j - V_j y_j.
\end{equation}
The angular distance between nonlinear and linear residuals can be computed by:
\begin{equation}
    d_j := 1 - \frac{(r^{nl}_j)^Tr^{lin}_j}{\|r^{nl}_j\|_2\cdot\|r^{lin}_j\|_2}.
\label{eq:switch}
\end{equation}
We set the threshold to 0.01. Thus, the linear update version will switch on when $d_j < 0.01$. We also check if $d_j \geq 0.01$ every short period, for example, every 10 iterations, to determine when we should switch back to the nonlinear version. Otherwise, we can set a fixed number of steps for a restart. This mechanism can significantly reduce the total number of function evaluations without sacrificing convergence and accuracy.

We use the Bratu problem to show the superiority of the adaptive update mechanism. The window size is $m=1$, and the starting point is an all-ones vector $x_0 = \textbf{1} \in \mathbb{R}^{10000}$. We use the relative norm of $f(x_j)$ as the cost/objective. In figure \ref{fig:bratu_mode_1}, we compare all three types of residual update in terms of the number of function evaluations. We see that the convergence rate of the adaptive update version is close to the linearized updated version without stagnation. The reason is that the adaptive update version switches to linear update at step 2 and changes back at step 110 where the linear update version becomes trapped. As for the cost (Y-axis) of each iteration, figure \ref{fig:bratu_mode_2} indicates that all three versions decrease almost the same per iteration before the stagnation happens. The adaptive update version performs as well as the nonlinear update version afterward. In what follows we default to adaptive nlTGCR unless otherwise clarified.

\subsubsection{Exploiting symmetry}
Recall that in the linear symmetric case, GCR is mathematically equivalent to the Conjugate Residual (CR) algorithm which is optimal with a window size of 1~\cite{Saad-Book2}. Our proposed nlTGCR also has this feature of using short term recurrence when the Jacobian is symmetric.

We tested nlTGCR along with a few baseline methods: Nesterov's Accelerated
Gradient~\cite{nesterov}, L-BFGS~\cite{liu1989limited}, AA, Nonlinear Conjugate
Gradient (NCG) of Fletcher\--Reeves' type~\cite{fletcher1964function}, and
Newton-CG~\cite{Dembo-al}. We analyze the convergence in terms of the number of
function evaluations rather than the number of iterations because the
backtracking line search is equipped for all considered methods except for AA by
default. The stopping criterion is relative residual
$\|F(s_k)\|_2/\|F(s_0)\|_2 < 10^{-16}$. The maximum number of iterations is
300. And the maximum number of steps for a restart is 50 if needed. The mixing
parameter for AA is set to $\beta = 0.1$ as suggested in
\cite{brezinski2022shanks}. For inexact Newton methods like Newton-CG and
Newton-GMRES, the restart means the maximum number of steps in the inner loop
that can be early terminated if
\begin{equation}
    \|r_k\| \leq \eta \|f(x_0)\|.
\end{equation}
We choose the forcing term $\eta = 0.9$ and adjust it via Eisenstat-Walker method~\cite{Eisenstat-Walker}.

\begin{figure}
      \parbox{0.48\textwidth}   {\includegraphics[width=0.48\textwidth]{Bratu_0.eps}
      \caption{The experiment of the Bratu problem at starting point $x_0 = \textbf{0}$. Each marker represents 10 iterations for all methods except Newton-CG (each marker represents 1 outer loop step).
      \label{fig:bratu_1}}}
      \hfill      
      \parbox{0.48\textwidth}   {\includegraphics[width=0.48\textwidth]{Bratu_1.eps}
      \caption{The experiment of the Bratu problem at starting point $x_0 = \textbf{1}$. Each marker represents 10 iterations for all methods except Newton-CG (each marker represents 1 outer loop step).
      \label{fig:bratu_2}}}
\end{figure}

The Jacobian $\nabla F(s)$ of the Bratu problem is symmetric positive definite (SPD). Therefore, nlTGCR with $m=1$ ought to get a good convergence. In contrast, methods that do not utilize the symmetry of Jacobian need more vectors to achieve similar performance. We consider two starting points: the starting point in figure \ref{fig:bratu_1} is an all-zeros vector $x_0 = \textbf{0}$ that is closer to the global optima, and the starting point in figure \ref{fig:bratu_2} is an all-ones vector $x_0 = \textbf{1}$. In both figures, we set the window size of L-BFGS and AA to 10, which indicates that 20 vectors in addition to $x_j$ and $r_j$ are stored, while nlTGCR only requires 2 extra vectors. In this problem, nlTGCR, Nesterov, Newton-CG, and NCG are memory efficient because they can store information on previous steps in only 1 or 2 vectors. Despite this, nlTGCR is still the fastest one.

      
\subsection{Molecular optimization with Lennard-Jones potential}

This problem illustrates the importance of exploiting the Jacobian of multiple points instead of using one Jacobian many times. The goal of geometry optimization is to find atom positions that minimize total potential energy as described by a certain potential.\footnote{Thanks: Stefan Goedecker's course site - Basel Univ. .. }
A potential that is commonly used is the Lennard-Jones (LJ) potential: 
\begin{equation}
        E = \sum_{i=1}^{N} \sum_{j=1}^{i-1} 4 \times
    \left[\frac{1}{\|x_i - x_j\|^{12}} - \frac{1}{\|x_i - x_j\|^{6}} \right]
\end{equation}
   In the above expression each $x_i$  is a 3-dimensional vector whose components are the coordinates of the location of
   atom $i$. In the experiment, we start with a certain configuration and 
   then optimize the geometry by minimizing the potential starting from that position. Note that the resulting position
   is not a global optimum - it is just a local minimum around some initial configuration. In this particular example,
   we simulate an Argon cluster by taking
   the initial position of the atoms to consist of a perturbed initial Face-Cented-Cubic structure \cite{meyer1964new}.
   We took 3 cells per direction - resulting in 27 unit cells. FCC cells include 4 atoms each and so we end up with a
   total of 108 atoms. 
   The problem is rather hard due to  the high powers in the potential. In this situation  backtracking or some form of
   line-search is essential.

\bigskip
      \fbox{ \parbox{0.2\textwidth}{Initial Config}}$\rightarrow$ 
     \fbox{ \parbox{0.35\textwidth}{Iterate to mininmize $\| \nabla E \|^2$}} $\rightarrow$ 
      \fbox{ \parbox{0.20\textwidth}{Final Config}}

\bigskip


The initial and final configurations are shown in Figure~\ref{fig:ArFig}.
\begin{figure}[htb] 
      \parbox{0.45\textwidth}{\includegraphics[width=.39\textwidth]{initGeom}}
      \parbox{0.08\textwidth}{$\longrightarrow$} 
      \parbox{0.45\textwidth}{\includegraphics[width=.39\textwidth]{finalGeom}}
      \caption{Initial (left) and final (right)  configurations of the 108 atoms with the Argon
        cluster experiment. \label{fig:ArFig}}
      \end{figure} 

In the following experiment, the vector $x_j$ is a vectorized array of coordinates of all atoms put together. So, it is a flat vector of length $3\times 108 = 324$.
We tested with AA, Nesterov, and Newton-GMRES. The reason for excluding L-BFGS, NCG, and Newton-CG is that the Jacobian $J(x_j)$ of the LJ problem is indefinite at some $x_j$. 
For example, we can verify that $J(x_0)$ is indefinite which can lead to a non-descending update direction.
Also, since nlTGCR and AA need to store $2m$ additional vectors to generate the searching subspace, the dimension of the subspace for Newton-GMRES is set to $2m$ so that all these methods are consuming the same amount of extra memory. 
The Newton-GMRES also has $\eta=0.9$ for early terminating the inner loop. AA does not converge unless the underlying fixed point iteration $x_{j+1} = x_j + \mu F(x_j)$ is selected carefully. 
Specifically, $\mu$ should neither be too large nor too small. For this reason, we choose $\mu = 10^{-3}$ in this experiment. 
The cost (Y-axis) is of the shifted potential $E - E_{min}$ where $E_{min}$ is the minimal potential achieved by all methods - which is close to $-579.4638$.

\begin{figure}[htb]
      \parbox{0.48\textwidth}{\includegraphics[width=0.48\textwidth]{LJ.eps}
      \caption{The experiment of the Lennard-Jones problem. Each marker represents 10 iterations for all methods except Newton-GMRES (each marker represents 1 outer loop step).\label{fig:LJ_1}}}
      \hfill
      \parbox{0.48\textwidth}{\includegraphics[width=0.48\textwidth]{LJ_zoomin.eps}
      \caption{Zoom-in of figure \ref{fig:LJ_1} that shows the performance near convergence.\label{fig:LJ_2}}}
\end{figure}

In figure \ref{fig:LJ_1}, we observe that nlTGCR with window size $m=10$ performs the best, especially when getting close to convergence. nlTGCR with window size $m=1$ and Newton-GMRES with subspace dimension 20 are close and slightly slower than nlTGCR (10). Another phenomenon worth discussing is that: if we look at the first few iterations, the inner loop of Newton-GMRES stops very soon. Therefore, Newton-GMRES doesn't focus on one Jacobian like it usually does. Instead, it moves to other Jacobians rapidly. This behavior explains why Newton-GMRES converges as fast as AA and nlTGCR do at the beginning. Indeed, the early stopping mechanism is essential to Newton-GMRES in this example, and we will discuss it next.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\textwidth]{LJ_base.eps}
    \caption{The experiment of the Lennard-Jones problem with base nlTGCR and fixed-inner-step Newton-GMRES.}
    \label{fig:LJ_base}
\end{figure}

Now we tested with the base nlTGCR and Newton-GMRES with a fixed number of inner steps, i.e., $\eta=0$. Here, we set the restart step to 20. The window size of nlTGCR is $m=1$ and $m=10$. The subspace dimension of Newton-GMRES is 5 and 10. As shown in figure \ref{fig:LJ_base}, when $m$ increases from 1 to 10, nlTGCR does not vary much as expected because the Jacobian is symmetric. But Newton-GMRES is getting less accurate and slower than nlTGCR at the beginning. The reason is that the Jacobian $J(x_j)$ can be very indefinite (both ends of the spectrum are far from 0). We know that nlTGCR uses the Jacobian of previous $m$ points to generate a new update direction. The weights of search directions $p_j$ will be computed in solving the least-square problem. Thus, the poor condition at one point will not heavily affect the overall convergence. However, Newton-GMRES uses the same $J(x_j)$ multiple times for each iteration. In other words, the update direction solely depends on $J(x_j)$. So, Newton-GMRES may not gain from performing more inner steps at one point in this example.


\subsection{Regularized logistic regression}
In this experiment, we show the performance of nlTGCR on optimization problems. The objective of the regularized logistic regression problem is to minimize $\phi(\theta)$ of the following form:
\begin{equation}
    \phi(\theta) = \frac{1}{N} \sum_{i=1}^N \log\left(1 + \text{exp}(-y_i \cdot x_i^T\theta)\right) + \frac{\lambda}{2} \|\theta\|_2^2
\end{equation}
where $x_i, y_i$ for $i=1,\dots,N$ are the training data and labels of Madelon
dataset~\cite{guyon2003design}.  There are 2000 samples, each of which has 500
features and a label of 1 or -1. We choose $\lambda = 10^{-2}$ in this
experiment. The starting point is $\theta_0 = 10^{-6}\cdot z$ where elements of
$z$ are drawn i.i.d. from the standard normal distribution. The maximum number
of iterations is 300, and the restart step is 40. The memory size is 10 for
nlTGCR, AA, and L-BFGS. In addition, AA uses $\beta=0.1$ and $\mu=10^{-5}$
because AA will explode immediately if using a larger $\mu$. For Newton-GMRES,
the subspace dimension is 20 for the same extra memory cost and the early
stopping parameter $\eta=0.9$.

\begin{figure}[htb]
      \parbox{0.48\textwidth}{\includegraphics[width=0.48\textwidth]{Reglog.eps}
      \caption{The experiment of the regularized logistic regression problem.  Each marker represents 10 iterations for all methods except Newton-GMRES (each marker represents 1 outer loop step).\label{fig:reglog_1}}}
      \hfill
      \parbox{0.48\textwidth}{\includegraphics[width=0.48\textwidth]{Reglog_zoomin.eps}
      \caption{Zoom-in of figure \ref{fig:reglog_1} that shows the performance at the beginning.\label{fig:reglog_2}}}
\end{figure}

Figure \ref{fig:reglog_1} and \ref{fig:reglog_2} show that nlTGCR converges fastest among all algorithms. Newton-GMRES is slightly slower than nlTGCR. Then it is followed by AA, L-BFGS, Nesterov, and NCG. The convergence speed of AA is restricted by $\mu$. That is to say, a greater $\mu$ usually leads to faster convergence. However, AA is sensitive to the choice of the starting point for this problem. For example, AA will not converge if $z$ is drawn from the standard uniform distribution on the interval $(0,1)$ unless we change the parameters. Other algorithms will not be affected if the perturbation on the starting point is small.



\subsection{Graph Convolutional Network}
This experiment demonstrates the potential of extending nlTGCR to DL problems as described in Section 4.8,. We consider applying graph convolutional networks (GCNs)~\cite{kipf2016semi} to the Cora dataset~\cite{mccallum2000automating}.

The Cora dataset contains 2708 scientific publications on one of 7 topics. Each publication is described by a binary vector of 1433 unique words indicating the absence or presence in the dictionary. This network consists of 5429 links representing the citation. The objective is a node classification via words and links. The neural network has one GCN layers with a dropout layer of rate 0.5.

\begin{figure}[htb]
    \centering
    \includegraphics[width=.95\textwidth]{GCN_Cora.png}
    \caption{nlTGCR vs. Adam: training loss and validation accuracy of GCN on the Cora node classification problem. Each marker represents 50 epochs.}
    \label{fig:Corafig}
\end{figure}

We considered the base version of nlTGCR with $m=1$ and $m=10$, and the restart is 15. Note that we do NOT use backtracking line search in this experiment. We also tested Adam~\cite{kingma2014adam} with learning rates $lr=0.01$ and $lr=0.001$. We can see from figure \ref{fig:Corafig} that nlTGCR shows competitive performance in this task. Specifically, it is not necessary to use a large window size since there is no significant difference between $m=1$ and $m=10$. So, the mat-vec computation cost can be small. Also, nlTGCR needs almost half the number of epochs as Adam needs to reach the same level of training loss that can mediate the drawback of having two function evaluations per iteration. This experiment shows as an example that we can adjust nlTGCR to solve DL problems. We will continue exploring other applications and techniques for stochastic situations.

\begin{comment}
\begin{table}[htp]
    \centering
    \begin{tabular}{l|l|l|l|l}
         Method & Train loss & Train acc & Val loss & Val acc \\
         \hline
         nlTGCR (lr=1.0) & 0.0788 & 1.00 & 0.8623 & \textbf{0.78} \\
         nlTGCR (lr=2.0) & \textbf{0.0576} & 1.00 & \textbf{0.8324} & \textbf{0.78} \\
         Adam (lr=0.01) & 0.1506 & 1.00 & 0.9908 & 0.75 \\
         Adam (lr=0.001) & 1.3510 & 1.00 & 1.6852 & 0.75 \\
    \end{tabular}
    \caption{nlTGCR vs. Adam: lowest loss and best accuracy achieved in 1000 epochs.}
    \label{tab:Cora_loss_acc}
\end{table}
\end{comment}






==> gcr.tex <==

\section{Nonlinear Truncated Generalized Conjugate Residual (nlTGCR) algorithm}\label{sec:linear} 
For understanding the conjugate residual-based methods in the nonlinear
case, it is important to first provide some background for
linear systems. A large
class of Krylov subspace methods for solving nonsymmetric linear systems have
been developed in the past four decades. The reader is referred to the recent
volume by Meurant and Tebbens \cite{Meurant-Tebbens} which contains a rather
exhaustive and detailed coverage of these methods.
The main aim of the techniques proposed in
this article is to  adapt the residual-minimizing
subclass of Krylov methods for linear systems to the nonlinear case.
The guiding principle in this adaption is that we 
would like it to also approximately minimize the
nonlinear residuals. This is in contrast with inexact Newton methods
where the goal is to roughly solve the linear systems that arise in
Newton's method as a way to provide a good search direction.

\subsection{The linear case:  Generalized Conjugate Residual (GCR) Algorithm}\label{sec:gcr} 
We first consider solving a linear system of the form: \eq{eq:Ax=b} A x = b .
\en A number of iterative methods developed in the 1980s aimed at minimizing the
norm of the residual $r = b -A x$ of a new iterate that lies in a Krylov
subspace, see \cite{Meurant-Tebbens} for a detailed account.  Among these, we
focus on the Generalized Conjugate Residual (GCR) algorithm \cite{Eis-Elm-Sch}
for solving \nref{eq:Ax=b} which is sketched in Alg. \ref{alg:gcr}.

\iffalse   
%%We will argue that the common approach of \emph{Inexact Newton Methods}
%%utilized in the past leads to some weaknesses.
%% YS TOO LONG + unnecessary
Solving the above system is equivalent to
   finding the  minimum of the quadratic form 
   $\phi_q(x) \equiv \half \| b - A x\|_2^2 $.
   %% The goal is to solve
   %% $\nabla \phi_q = 0$, which leads to the linear system $Ax=b$.
Here, the gradient of $ \phi_q(x)$  is
$A^T (Ax-b)$ and its Hessian is the matrix $A^T A $.
However, standard methods based on this framework tend to be slow because
the condition number of $A^T A$ is usually large. As a result,
researchers developed methods based on using the standard residuals
$ r = b -A x$ to search for the minimum. For example,  the Generalized Conjugate Residual (GCR)
algorithm \cite{Eis-Elm-Sch} 
for solving \nref{eq:Ax=b} can formally be described as
shown in Alg. \ref{alg:gcr}.
\fi

%% 
    \begin{algorithm}[htb]
    \centering
    \caption{GCR}\label{alg:gcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: Matrix $A$, RHS $b$,
  initial  $x_0$. \\
  Set $p_0=r_0 \equiv b-Ax_0$.
\For{$j=0,1,2,\cdots,$ until convergence} 
\State  $\alpha_j =  \langle r_j, A p_j \rangle / \langle A p_j, A p_j\rangle $
\State $x_{j+1} = x_j + \alpha_j p_j$
\State $r_{j+1} = r_j - \alpha_j A p_j$
\State $p_{j+1} = r_{j+1} - \sum_{i=0}^j \beta_{ij} p_i $ \quad where \quad
$\beta_{ij} :=  \langle A r_{j+1} , Ap_i\rangle / \langle A p_i, Ap_i\rangle $
\EndFor
\end{algorithmic}
\end{algorithm}
The main point of the algorithm is to build a sequence of search
directions $p_i$, $i=0:j$ at step $j$ so that the vectors $A p_i$ are
orthogonal. This is done in Line~7.  With this we know that the
iterate as defined by Lines 4-5 is optimal in the sense that it yields
the smallest residual norm among solution vectors selected from the
Krylov subspace $x_0 + \mbox{span}\{p_0, \ldots, p_k\}$ -- see \cite[pp 195-196]{Saad-Book2}.  The GCR
algorithm is mathematically equivalent
\footnote{Here equivalent is meant in the sense that if exact arithmetic is
  used and if the compared algorithms both succeed in  producing the $j$-th
  iterate from the same initial $x_0$, then the two iterates are equal.} 
to GMRES~\cite{Saad-book3}, and
to some of the forms of other methods developed earlier, e.g.,
ORTHOMIN~\cite{Vinsome76}, ORTHODIR~\cite{Jea-Young}, and Axelsson's
CGLS method \cite{Axelsson80}.  
%A detailed account of Krylov subspace methods for nonsymmetric linear systems and their inter-relationships
%can be found in the exaustive treatise by Meurant and Duintjer
%Tebbens~\cite{Meurant-Tebbens}.

\iffalse
Eisenstat, Elman and Schultz established
a number of results including convergence for the situation when
$A$ is positive real, i.e., when the symmetric part of $A$ is positive
definite. Among other properties of the algorithm shown
are the orthogonality of the directions $Ap_i$, and the fact that
the iterate
$ x_{k+1}$ minimizes the residual norm over
$x_0 + \mbox{span}\{p_0, . . . , p_k\}$.
The orthogonality of the vectors $Ap_i$  is equivalent to the property that 
the directions $p_i$ are $A^TA$-orthogonal.
Another property of GCR  is that the 
residual vectors that it produces  are
`semi-conjugate' in that $ (r_i, Ar_j ) = 0$ for $i > j$.
\fi



\iffalse
the following theorem
- \cite{Eis-Elm-Sch}:
\begin{theorem}\label{thm:gcr}
  The following properties are satisfied by the vectors produced by
  Algorithm~\ref{alg:gcr}
\begin{enumerate}
\item $ (Ap_i, Ap_j ) = 0,$ for $ i \ne j$,
\item $ (r_i, Ap_j ) = 0,$ for $ i > j$,
\item $ (r_i, Ap_i  ) = (r_i, Ar_i )$,
\item $ (r_i, Ar_j ) = 0, i > j$,
\item $ (r_j , Ap_i ) = (r_0, Ap_i ), i \ge j$,
\item $ \{p_0, . . . , p_{k-1} \}$ and $\{r_0, . . . , r_{k-1} \} \
\mbox{span} \ K_k (A, r_0 )$, 
\item $ x_{k+1}$ minimizes the residual norm over $x_0 + \mbox{span}\{p_0, . . . , p_k\}$.
\end{enumerate}
\end{theorem}
\fi

Next we will discuss a truncated version of GCR
in which the $Ap_i$'s are only orthogonal to the $m$ previous
ones. This algorithm was first introduced by Vinsome as early as in 1976
and was named `ORTHOMIN' \cite{Vinsome76}. We will just refer to it as
the truncated version of GCR or TGCR.
%%Indeed it is unrealistic to keep all $A p_i$ vectors as this could require
%%an excessive amoumt of memory.
In what follows we will also write the algorithm in a form that is closer to a
practical implementation. Indeed, at step $j$ we need to keep a set of $m$ vectors
for the $p_i$'s and the other set for the vectors $v_i = A p_i$.  In addition, the orthogonalization in Line~7 is a form of
classical Gram-Schmidt which we can replace by the modified form of Gram-Schmidt by
setting the vector $A r_{j+1} $ initially to a vector $v$ which is
orthogonalized against the successive $A p_i$'s.  The resulting truncated GCR
algorithm is a slight variant of the original ORTHOMIN algorithm introduced 
in \cite{Vinsome76} and analyzed in  \cite{Eis-Elm-Sch}.
%%A number of methods were developed in the
%%1980s 1990s that were relatively close to each other, see \cite{Meurant-Tebbens}
%%for details.
  
\begin{algorithm}[htb]
  \centering
  \caption{TGCR(m)}\label{alg:tgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: Matrix $A$, RHS $b$,
  initial  $x_0$. \\
  Set $r_0 \equiv b-Ax_0$; $v = A r_0$; 
  \State $v_0 = v/\| v \|$;   $p_0 = r_0 / \| v \|$; 
\For{$j=0,1,2,\cdots,$ Until convergence} 
\State  $\alpha_j = \langle r_j, v_j\rangle $
\State $x_{j+1} = x_j + \alpha_j p_j$
\State $r_{j+1} = r_j - \alpha_j v_j$
\State $p = r_{j+1}$;  \quad  $ v = A p $;   \quad  and  \quad  $j_m = \max(0,j-m+1)$  
\For{$i=j_m:j$} 
\State $\beta_{ij} :=  \langle v, Ap_i \rangle $
\State $p := p - \beta_{ij} p_i$;
\State  $v := v - \beta_{ij} v_i$; 
\EndFor
\State $p_{j+1} :=p /\| v\|$ ; \qquad  $v_{j+1} :=v/\|v\|$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}

As is seen in Line 3 and Line 14, we normalize each $v_i $ so $\| v_i \|=1$
and $p_i$ is normalized accordingly.
Steps 9--14 of the algorithm produce  a system of 
vectors 
$V_{j+1} = [v_{j_m}, v_{j_{m}+1},\ldots,v_j, v_{j+1}]$ that is orthonormal.
When $j \ge m$, $V_{j+1}$ consists of a `window' of $m+1$ vectors. Algorithm \ref{alg:tgcr} can be viewed as a method for approximately minimizing
the quadratic form $\phi_q(x) \equiv \half \| b - A x\|_2^2 $ in
a certain Krylov subspace.
With $m = \infty $ we obtain the non-restarted GCR method - which is equivalent to the non-started GMRES \cite{Saad-book3}.
The purpose of  Lines 8 to 14 is to compute the new direction $p_{j+1}$ --
by ortho-normalizing the vector $Ar_{j+1}$ against all previous $Ap_i$. From Line~11, we obtain
the relation $A p_{j+1} = A r_{j+1} - \sum_{i=j_m,j}  \beta_{ij}Ap_i$
from which it becomes clear that
$A p_{j+1} \perp A p_i $ for $i=j_m, \ldots,j$.


\iffalse
The properties in the next theorem were written in a slightly different form in
~\cite[Th. 4.1]{Eis-Elm-Sch}.
\begin{theorem}\label{thm:tgcr} 
  The following properties are satisfied by the vectors produced by
  Algorithm~\ref{alg:tgcr}
  \begin{enumerate}
\item  $(Ap_{j+1}, A p_i) = 0$, for $i = j_m,\ldots, j $ 
\item   $(r_{j+1}, Ap_i) = 0,$ for $ i=(j-1)_m,\ldots,j.$ 
\item  $(r_j, Ap_j) = (r_j, Ar_j)$,
\item  $(r_{j+1}, Ar_j) = 0$,
\item  $(r_j, Ap_i) = (r_{i-m}, Ap_i), j=i-m, \cdots,i, i \ge m$,
\item  if $r_i \ne 0$, then $p_i \ne 0$, \textcolor{blue}{YX: This property requires $A$ to be positive definite.}
\item  for $i \ge m, x_{i+1}$ minimizes $\|b - Ax\|_2$ over the space
                              $x_{i-m} + \mbox{span} \{p_{i_m},\cdots p_i\}.$
\end{enumerate}
\end{theorem} 
\fi
                           
A few properties of the vectors generated in TGCR(m) have been analyzed in
~\cite[Th. 4.1]{Eis-Elm-Sch} which  also discussed the convergence of the algorithm
when $A$  is positive definite, i.e., when $A+A^T$ is symmetric positive definite.
When $A$ is symmetric a number of simplifications
take place in Algorithm ~\ref{alg:gcr}. 
In this situation,   all the $\beta_{ij}$'s except 
$\beta_{jj} $ vanish. 
\iffalse 
In this situation, 
that all the $\beta_{ij}$'s except 
$\beta_{jj} $ which we now denote by $\beta_j$.  See Proposition \ref{prop:cr} for the proof.

%%(in analogy with notation in CG). 
As a result
Algorithm~\ref{alg:gcr} simplifies:  Line 1-6 remain unchanged and
Line~7 is replaced by: 
\bigskip
\betab
\>7.cr:  \> \>
$p_{j+1} = r_{j+1} - \beta_{j} p_j $ \quad where \quad
$\beta_{j} :=  \langle A r_{j+1} , Ap_j\rangle / \langle A p_j, Ap_j\rangle $  .
\entab
\bigskip

The following alternative expressions for the scalars
$\alpha_j$ and $\beta_j$, that resemble those of the CG algorithm,
can be easily established 
%%by exploiting well-known properties of GCR:
\eq{eq:NewGCR}
\alpha_j = \frac{ \langle r_j, A r_j\rangle }{ \langle A p_j, A p_j\rangle } \qquad
\beta_j = - \frac{\langle A r_{j+1} , r_{j+1}\rangle }{\langle A r_j, r_j\rangle } . 
\en
\fi
The resulting simplified algorithm yields the standard Conjugate Residual (CR)  algorithm
which dates back to Stiefel \cite{Stiefel-CR}, see
\cite[sec 6.8]{Saad-book3} for details.
\iffalse
These expressions are those used in the usual
  way of defining the Conjugate Residual (CR) algorithm 
  The CR Algorithm 
\fi
 
  \subsection{The nonlinear extention: nonlinear TGCR (nlTGCR) algorithm}\label{sec:nonlin}
  We now return to the nonlinear problem and ask the question:  how can we
  generalize the algorithms for linear systems of Section~\ref{sec:gcr} for solving nonlinear
  equations? We should begin by stating what are the desired features of this
  extension.
  First we would like the algorithms to  fall back to TGCR when the problem is linear.
  Second, we would like a method that can be adapted in such a way as to yield
  the inexact Newton viewpoint when desired or a multi-secant (AA-like) approach when
  desired. Third, we would like a method that exploits a more accurate linear model than
  either Newton or a quasi-Newton approach - possibly at the cost of  a few extra function
  evaluations. Finally, we would like the algorithm to be easily adaptable to the very
  common context in which the function $f$ is `fuzzy' as is the case when dealing with
  stochastic methods. 
  


\iffalse
  If there is no
  ambiguity we will denote $J(x_j)$ by $J$.  Note that the right-hand side of
  the Newton system is $-f(x_j)$ and this is also the residual for $x_j$, i.e.,
  when $\delta_j = 0$.
%  iterative refinement in the 
%  linear case where the right-hand side is the residual,
  Therefore, we will define the residual vector $r_j$  to  be $r_j = -f(x)$.
\fi 

  
  
  In our model we assume that at step $j$ we have a set 
  of (at most) $m$ current `search' directions
  $\{ p_i \} $ for $j_m \le i \le j$  gathered as columns of a matrix $P_j$,
  where we recall the notation $j_m \equiv \max\{0,j-m+1 \}$.
  Along with each $p_i$ we also assume that $v_i \equiv J(x_i) p_i $ is
  available and also   saved in a matrix denoted by $V_j$, so that
    \eq{eq:PjVj}
    P_j = [ p_{j_m}, p_{j_m+1},\cdots, p_j],
    \qquad 
    V_j = [ v_{j_m}, v_{j_m+1},\cdots, v_j].
    \en
    Note that this pair of matrices plays the same role as does the pair
    $\XX_j, \ \FF_j$ defined in \eqref{eq:dfdx} for Anderson acceleration.
  We then  write the linear model used locally as 
   \eq{eq:nltgcrmodle} f(x_j + P_j y) \approx f(x_j) + [J] P_j y \en where $[J] P_j$
  should be interpreted as \eq{eq:JP} [J] P_j \equiv [ J(x_{j_m})
  p_{j_m}, \cdots, J(x_{j}) p_{j} ] = V_j , \en
  i.e.,  the Jacobian  applied to each vector $p_i$ is calculated
  at the point $x_i$ and is therefore different for each $i$.
  While this is again somewhat similar to what was done for Anderson
  acceleration, we note a very important distinction that may have
  a siginificant effect on performance: \emph{In Anderson acceleration
    the linear model is simply based on the relation
    $f(x_j-\XX_j \theta) \approx f(x_j) -\FF_j\theta$ whereas nlTGCR evaluates
    explicitly  $J(x_i) p_i $.} This evaluation can be quite accurate if desired.
  In contrast, the relation
  $f(x_j-\XX_j \theta) \approx f(x_j) -\FF_j\theta$ can be quite rough,
  especially at the beginning of the process where the vectors $\Delta x_j$ and
 $\Delta f_j$ are not small.    
  
  The projection method will minimize the norm
  $\| f(x_j) + [J] P_j y \|_2 = \| f(x_j) + V_j y \|_2 $. This is achieved
  by determining $y$ in such a way that
  \eq{eq:opt} f(x_j) + V_j y \perp \Span \{V_j\} \
  \rightarrow \ (V_j)^T[f(x_j) + V_j y] = 0 \ \rightarrow \ y = 
  V_j^T r_j
  \en
  where it is assumed the $v_i$'s are orthonormal.
  \iffalse Note that in the linear case, it can be shown that
  $v_i^T r_j = 0 $ for $j_m \le i < j$, so that $V_j^T r_j$ has only
  one nonzero component. The assumption that the $p_i$'s are fully
  orthogonal implies that $j_m$ is always equal to one.  In the
  situation we have partial orthogonality ($j_m > 1$) -- we can solve
  the least-squares problem explicitly instead of exploiting
  orthogonality.  A simpler alternative is just to redefine $P_j$ and
  $V_j$ to consist of their columns $j_m $ to $j$ which are
  orthogonal.
\fi 
    
  
Instead  of (\ref{eq:inex1}--\ref{eq:inex2}) of the inexact Newton approach
we now have an iteration of the form
    \begin{align} 
 &      \mbox{Find}  & y &= \mbox{argmin}_y \| f(x_j) + V_j y \|_2 &  \label {eq:inex3}\\
 &       \mbox{Set}  & x_{j+1}  & = x_j + P_j y_j & \label {eq:inex4}
  \end{align}  
  A major distinction between this approach and standard inexact
  Newton is that the latter exploits approximations to the Jacobian
  around one point in order to build the next iterate.  The iterates
  generated by the iterative process can be viewed as intermediate
  points but they rely on an a Jacobian calculated $J(x_0)$ at the initial
  approximation.
  %%Thus, intermediate iterates do not use updated
  %%versions of the Jacobian.
  We will revisit the inexact Newton viewpoint in a  later   section.

  \iffalse 
  The proposed approach uses $m$ pairs of vectors $p_i, J(x_i) p_i$.
  %% and as was already mentioned
 these pairs resemble the pairs $\Delta x_j, \Delta f_j$ of AA.
 However, in our case, computing $J(x_i) p_i$  comes at the cost of
 doubling the number of function evaluations,
 although  the local model is likely to be more accurate and this could be
 more important at the beginning of the process. 
 \fi
 
   The idea of the nonlinear version of the truncated GCR method is to
   exploit the directions that are produced by the TGCR algorithm.
   Note here is that there is a decoupling between the \emph{update}
   from the current iterate to a new one (Lines 5--6) and the
   \emph{construction of the $p_i$'s} in TGCR (Lines 8--14).  In
   essence, the first part just builds a new approximation given a new
   `search' subspace - while the second adds a new direction to this
   evolving subspace, by exploring the most recent residual (Line
   8).
   This distinction will help us generalize our approach to cases where
   the objective function or the Jacobian varies as the iteration proceeds.
   
   %% In the nonlinear case, we must take this residual to be the   nonlinear one.

    \begin{algorithm}[htb]
    \centering
    \caption{nlTGCR(m)}\label{alg:nltgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: $f(x)$,   initial  $x_0$. \\
  Set $r_0 = - f(x_0)$.
  \State Compute  $v = J(x_0)  r_0$; \ (Use Frechet)
  \State $v_0 = v/ \| v \| $, $p_0 = r_0/ \| v \|_2 $;
  \For{$j=0,1,2,\cdots,$ } 
\State  $y_j = V_j^T r_j $ 
\State $x_{j+1} = x_j + P_j y_j$
\State $r_{j+1} = -f(x_{j+1}) $ 
\State Set: $p := r_{j+1}$; and $j_m = \max(0,j-m+1)$
\State Compute $v =  J(x_{j+1})  p$ (Use Frechet)
\For{$i=j_m:j$}
\State $\beta_{ij} :=  \langle v, v_i \rangle $
\State $p := p - \beta_{ij} p_i$
\State $v := v - \beta_{ij} v_i$
\EndFor
\State $p_{j+1} :=p /\| v\|_2$ ; \qquad  $v_{j+1} :=v/\|v\|_2$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}


  
  We now derive our general algorithm from which a few variants will follow.
  The algorithm is an extension of Algorithm~\ref{alg:tgcr} -- with a few
  needed changes that reflect the nonlinearity of the problem.
  The first change is that any residual is now to be replaced by the negative of
  $f(x)$ so  Line~2 of Algorithm~\ref{alg:tgcr} becomes
  $r_0 = -  f(x_0)$ and Line~7 must be replaced by
  $r_{j+1}  = -  f(x_{j+1})$. In  addition, the matrix $A$ in   the 
  products  $A  r_0  $  and  $A  p$ invoked  in    Line~2  and  Line~8
  respectively, is the   Jacobian of  $f$ at the most recent 
  iterate.  The most
  important  change is  in  Lines  6-7 where  according  to the  above
  discussion the scalar $\alpha_j$  of Algorithm~\ref{alg:tgcr} is to be replaced
  by the 
  vector $y_j$ that  minimized $\| f(x_j) + V_j y \|_2$ over $y$.
  The reason for this was explained above.  
%%    $(v_j ,v_i) = \delta_{ij} \quad \mbox{for}\quad j_m \le i \le j $

  
The resulting algorithm is shown in Algorithm~\ref{alg:nltgcr}.  
It requires two function evaluations per step : one in Line 8 and the
other in Line~10.  In the situation when computing the Jacobian is
inexpensive, then one can compute $J p$ in Line~10 as a matrix-vector
product. Apparently, the system $[v_{j_m}, v_{j_m +1}, \cdots,  v_{j+1}] $ is orthonormal. 
%and this will reduce the number of function evaluations per step from 2 to 1.
%% Next we examine properties ..

  
\section{Theoretical results}
This section discusses connections of nlTGCR algorithm with inexact and quasi-Newton methods
and analyzes  its convergence.
\subsection{Linearized update version and the connections to inexact Newton methods} 
\label{sec:LinUpd} 
We first consider a variant of the algorithm which we call
the ``linearized update version''. We will show that this version is equivalent to inexact Newton methods in which the system is approximately solved with TGCR. Two changes are made to Algorithm \ref{alg:nltgcr} to obtain this linearized update version. 
First,  in Line~8 we update the
residual by using the linear model, namely, we replace Line~8 by: 
 
\bigskip
%%\hrule
\betab
\> 8a:  \> \>  $ r_{j+1} = r_j - V_j y_j$
\entab
\smallskip 


%% In addition, in order to obtain the exact equivalent of
%% inexact Newton methods,

The second change is that the Jacobian is not updated in Line~10, i.e.,
$J(x_{j+1})$ in Line 10 is kept constant
and equal to $J(x_0)$. In other words
$v$ is computed as
\bigskip
\betab
\> 10a:  \> \>   $ v = J(x_0) p $ 
\entab
\smallskip 

%%If $k$ steps of the algorithm are carried out we would get what amounts to
%%When $F$ is linear, then the residual at step $j+1$ becomes
%%$r_{j+1} = b - A(x_j + P_j y_j) = r_j - A P_j y_j $ and we recall that
%%$Ap_i$ is saved as $v_i$.
%% In addition, in order to obtain the exact equivalent of
%% inexact Newton methods, the Jacobian $J$ in Line 10 is kept constant
%% and equal to $J(x_0)$.

The algorithm is stopped  when the residual norm $r_{j+1} $
is small enough or the number of steps is exceeded.
In addition, \emph{we consider the algorithm merely as a means of providing
  a search direction} as is often done with inexact Newton methods.
In other words the direction $d = x_{last} - x_0$ is provided
to another function which will use it in an iterative procedure
which will include a linesearch technique at $x_0$. 

It is easy to see that one iteration defined as a sweep using $j$ substeps of
this linear update version is nothing but \emph{an inexact Newton method in
  which the system \nref{eq:inex1} (with $j=0$) is approximately solved with the
  TGCR algorithm.}  Indeed, in this situation Lines 4-15 of
Algorithm~\ref{alg:tgcr} and Lines 5-17 of Algorithm~\ref{alg:nltgcr} are
identical.  Lines 5-17 of Algorithm~\ref{alg:nltgcr} perform $k$ steps of the
TGCR algorithm to solve the linear systems $f(x_0) + J(x_0) P y = 0$.  Within
Algorithm~\ref{alg:nltgcr} the update is written in progressive form as
$x_{j+1} = x_j + \alpha_j p_j$, note that \emph{the right-hand side does not
  change during the algorithm and is equal to $r_0 = - f(x_0)$.  } In effect the
last iterate, $x_k$, is updated from $x_0$ by adding a vector from the Krylov
subspace or equivalently the span of $P_k$.  As a consequence of this
observation, it turns out that $y_j$ has only one nonzero component, namely the
last one.  Indeed, from ~\cite[Th. 4.1]{Eis-Elm-Sch}, we see that if we replace
$A$ by the Jacobian $J$ at $x_0$ then:
\[
  \langle r_{j+1}, J p_i\rangle = 0  \ \mbox{for} \ i=(j-1)_m, \cdots, j. 
\]

It was shown in \cite{Brown-Saad} that under mild conditions, the update to the
iterate is a descent direction. In addition, the article describes `global
convergence strategies' based on linesearch and trust-region techniques.  If we
do not apply a global convergence strategy, then the algorithm may have difficulties
to converge.


Inexact Newton methods \cite{Dembo-al} 
are often implemented with residual reduction stopping criteria of the form
\eq{eq:forcing}
\| f(x_j) + J(x_j) \delta_j \|_2 \le \eta_j \| f(x_j) \|_2
\en
where  $\eta_j \in [0,1) $ is called the forcing term.
This only means that the iterative procedure that is applied when
approximately solving the linear system \nref{eq:inex1} exits when
the relative residual norm falls below $\eta_j$.
A number of articles established convergence conditions under conditions
based on this framework, see, e.g.,
\cite{Dembo-al,Brown-Saad,Brown-Saad2,Eisenstat-Walker94} among others. 

%%As was already mentioned, inexact Newton methods have a number of
%%disadvantages.
Probably the most significant disadvantage of inexact Newton methods
is that a large 
number of function evaluations may be needed to build the Krylov
subspace in order to obtain a single iterate, i.e., the  next  iterate. 
After this iterate is computed, all the information gathered at
this step, e.g., $P_k, V_k$, is discarded. This is to be contrasted with
quasi-Newton techniques where the most recent function evaluation
contributes to building an updated approximate Jacobian.

\subsection{Nonlinear update version}
The ``linearized update version" of Algorithm~\ref{alg:nltgcr} discussed above uses
a simple linear model to update the residual $r_j$ in which the Jacobian is not updated.
Next, we consider the ``nonlinear update version" as described in
Algorithm~\ref{alg:nltgcr}. %This version explicitly enforces the linear
%optimality condition of GCR, as represented by Equation~\nref{eq:opt}.

Assume a sweep using
$j$ substeps of Algorithm~\ref{alg:nltgcr} has been carried out. Our next result will invoke the  linear residual
\eq{eq:LinRes} \tilde r_{j+1} = r_j - V_j y_j , \en
as well as the deviation between the actual residual $r_{j+1}$ and its
linear version $\tilde r_{j+1}$ at the $j+1$th iteration: 
\eq{eq:ResDev} z_{j+1} = \tilde r_{j+1} - r_{j+1} . \en 

 
We first analyze the magnitude of $z_{j+1}$. Define
\eq{eq:wi}
w_i = (J(x_j) - J(x_i)) p_i \ \mbox{for} \ i=j_m, \cdots, j ;  \quad \mbox{and}\quad 
W_j = [w_{j_m}, \cdots, w_j ].
\en
%% ---- delta_j --> s_j
Observe  that
\eq{eq:Jxjpi}
  J(x_j) p_i = J(x_i) p_i + w_i = v_i + w_i .
  \en
  We also define:
\eq{eq:2ndOrd}
s_j  = f(x_{j+1}) - f(x_j) -  J(x_j) (x_{j+1} - x_j) . 
\en
Recall  from the Taylor series expansion $s_j$ is a second order term relative
to $\| x_{j+1}-x_j \|_2$. 
Then we derive the following bound on the norm of $z_{j+1}$ in the next proposition.


\begin{proposition}\label{prop:2}
  The difference $\tilde r_{j+1} - r_{j+1} $ satisfies the relation:
\eq{eq:ResDiff}
\tilde r_{j+1} - r_{j+1}  =   W_j y_j  + s_j
=   W_j V_j^T r_j  + s_j ,
\en
and therefore:
\eq{eq:ResDiffN}
\| \tilde r_{j+1} - r_{j+1} \|_2   \le \| W_j \|_2  \ \| r_j \|_2 + \| s_j \|_2 . 
\en

\end{proposition}

\begin{proof} 
We rewrite the difference as:
\begin{align}
  \tilde r_{j+1} -r_{j+1}
  & = (-f(x_j) - V_j y_j ) + f(x_{j+1})  \nonumber\\
  & = (f(x_{j+1}) - f(x_j))  - V_j y_j  \nonumber\\
  & = J(x_j) P_j y_j + s_j - V_j y_j \label{eq:prop2pf}
\end{align}       

Letting $ y_j = [ \eta_1, \eta_2, \cdots ]$ we  get
\begin{align}
  J(x_j) P_j y_j
  &= \sum  \eta_i J(x_j) p_i  \nonumber \\
  &= \sum \eta_i J(x_i) p_i   + \sum \eta_i (J(x_j) -J(x_i)) p_i \nonumber\\
  &= V_j y_j  + W_j y_j . \label{eq:prop2pf2} 
  \end{align}
The proof follows by combining \eqref{eq:prop2pf} and \eqref{eq:prop2pf2} \end{proof}
 
The proposition shows that $z_{j+1}$ is a quantity of the second order:
when the process is nearing convergence, 
$\| W_j \|_2 \| r_j \|_2 $ is the product of two first order terms
while $s_j$ is a second
order term according to its  definition \nref{eq:2ndOrd}.
\iffalse
Let us explore this a little further by making the assumption that:
 \eq{eq:2ndOrd1}
 \| (J(y) - J(x)) p  \|_2 \le   L_h \|x-y\|_2 \ \| J(x) p \|_2 . 
 \en
 Recalling that $\|J(x_i)  p_i \|_2 = \|v_i \|_2 = 1$, we get

 \eq{eq:wibnd} 
   \|w_i \|_2 = \| (J(x_j) - J(x_i)) p_i\|_2 \le
   L_h \| x_j - x_i \|_2 \| J(x_i)  p_i \|_2 =       L_h \| x_j - x_i \|_2
   \en
      and it follows from \nref{eq:wibnd} that
  \[
   \| W_j\|_2\| r_j \|_2 \le  m_j L_h \times \frac{1}{m_j} \sum \|x_i - x_j \|_2  \ \| r_j \|_2 \]
  The term
 \[  \frac{1}{m_j} \sum \|x_i - x_j \|_2  \equiv \rho_j \]
 denotes the average distance from the previous $m_j$ iterates
 $x_i $ to $x_j$. Thus, we have 
 \eq{eq:bndWr}
 \|W\|_2  \| r_j \|_2 \le m_j L_h \rho_j \|r_j\|_2 .
 \en
 When the process is nearing convergence, the right-hand side is clearly
 a second-order term.
 \fi
 Furthermore, we can prove the following properties of Algorithm~\ref{alg:nltgcr}.
\begin{proposition}\label{prop:nltgcr} 
    The following properties are satisfied by the vectors produced by
    Algorithm~\ref{alg:nltgcr}:
    %% where $e_{1,k} $ is the $1$st column of the identity matrix    of dimension $k$.
    

  \begin{enumerate}
 

  \item 
    $ ( \tilde r_{j+1}, v_i) = 0  \quad \mbox{for} \quad j_m \le i \le j$,
    i.e., $V_{j}^T \tilde r_{j+1} = 0$;

    
  \item 
    $ \| \tilde r_{j+1} \|_2 = \min_y \| -f(x_j) + [J] P_j y\|_2
    = \min_y \| -f(x_j) + V_j y\|_2 $;

    
  \item $\langle v_{j+1} , \tilde r_{j+1}\rangle
    = \left \langle v_{j+1} \ , r_j \right \rangle $;

  \item $y_j=V_{j}^T r_{j} = \langle v_{j}, \tilde r_{j} \rangle e_{m_j} - V_{j}^T z_{j}  $
    where $ e_{m_j} = [0, 0, \cdots, 1]^T \in \ \RR^{m_j}$.
    
%%  \item $V_{j}^T r_{j} = (v_{j}, \tilde r_{j}) e_{1,m_j} + V_{j}^T z_{j}  $
%%    where $ e_{1,m_j} = [1, 0, \cdots, 0]^T \in \ \RR^{m_j}$ with $m_j = \min \{m, j+1\}$.

\end{enumerate}

\medskip 
\end{proposition}

\begin{proof} 
  Properties (1) and (2) follow from the definition of the algorithm.
  For Property (3)  first observe  that
  $V_j = [v_{j_m}, v_{j_m+1},\cdots, v_{j-1}, v_j]$
  and that $v_{j+1}$ is made orthogonal against  the $m_j$ vectors    $v_{j_m}$ to $ v_j$,
  so $ v_{j+1}^T  V_j  = 0 $ and
  \[
  v_{j+1}^T  \tilde r_{j+1}   =  v_{j+1}^T [r_j - V_j y_j]
  \ = \   v_{j+1}^T r_j . 
  \]

  It is convenient to prove  Property (4)  for the index $j+1$ instead of $j$. We write:
  $     V_{j+1}^T r_{j+1} =  V_{j+1}^T [\tilde r_{j+1} - z_{j+1} ] $ 
where $z_{j+1} $ was defined in Equation \eqref{eq:ResDev}.
  Recalling Properties (1) and (3), we have that
  $\langle \tilde r_{j+1}, v_i \rangle = 0 $ for $j_m \le i \le j$ - so there is only one nonzero term
  in the product $V_{j+1}^T \tilde r_{j+1}$, namely  $v_{j+1}^T \tilde r_{j+1}$.
 \iffalse i.e.,
  \[   \tilde r_{j+1}^T V_{j+1}
  = \tilde r_{j+1}^T [v_{(j+1)_m}, \cdots,  v_j, v_{j+1} ]
  = [0, 0 , \cdots, 0,   \tilde r_{j+1}^T v_{j+1} ]
  = \tilde r_{j+1}^T v_{j+1} e_{k}^T 
\]
where $e_k \ \in \ \RR^k$ and
$k$ is the number of columns in $V_{j+1}$, which is $\min \{m, j+2\}$
(recall: indexing starts at $j=0$ so $V_{j+1}$ has $j+2$ columns when $j+2\le m$).
\fi
This gives the results after adjusting for the change of index.
\end{proof}   

Property (4) and Proposition \ref{prop:nltgcr} indicate that when $z_j$ is small, as when the model is \emph{close to being linear} or when it is nearing convergence,
then  $y_{j} $ will have small components everywhere except for the last component. 
As a result it is also possible to consider a slight variant of the algorithm in which  $y_j$ is truncated so as to contain only its last entry.  We will discuss this variant in detail in Section \ref{subsec:linesearch}.


 
 \subsection{Connections to quasi-Newton and multi-secant methods} 
In this section, we show that nlTGCR can be viewed from the alternative angle of
a quasi-Newton/multi-secant approach. In this viewpoint,  the inverse of the Jacobian
is approximated progressively. Because it is the inverse Jacobian that is
approximated, the method is akin to Broyden's second update method.

First  observe that in nlTGCR  the update at step $j$ takes the form:

\[x_{j+1} = x_j + P_j V_j^T r_j = x_j + P_j V_j^T (-f(x_j)) . \]
Thus, we are in effect using a secant-type method.
The approximate inverse Jacobian at step
$j$,  denoted by  $G_{j+1} $ for consistency with common
notation, is: 
\eq{eq:Gj}
G_{j+1} = P_j V_j^T .
\en 
If we apply this to $v_i$ we get
$
  G_{j+1} v_i = P_j V_j^T v_i =  p_i =  J(x_i) \inv v_i \quad \mbox{for} \quad j_m \le i \le j.
$ 
So $G_{j+1}$ inverts $J(x_i)$ exactly when applied to $v_i$. It therefore satisfies 
the \emph{secant} equation
\eq{eq:msecant1} 
  G_{j+1} v_i = p_i \quad \mbox{for} \quad j_m \le i \le j,
  \en
which is a version of \nref{eq:secant2}   used in    Broyden's second update method.
Here,  $p_{i}$ plays the role of $\Delta x_j$ and $v_i$ plays the role
  of $\Delta f_j$.
In addition, the update $G_{j+1}$ satisfies the `no-change' condition:
\eq{eq:msecant2} 
  G_{j+1} q = 0 \quad \forall q \perp v_i  \quad \mbox{for} \quad j_m \le i \le j.
  \en
  The usual no-change condition for secant methods is of the form
  $(G_{j+1}-G_{j-m}) q = 0 $ for $q \perp \Delta f_i$ which in our case
  would be
  $(G_{j+1}-G_{j-m}) q = 0 $ for $q \perp \ v_i  \quad \mbox{for} \quad j_m \le i \le j$.
  One can  therefore consider that we are updating $G_{j-m} \equiv 0$.




  Thus, consider the optimization problem
  \eq{eq:optB}
  \min \{  \| G \|_F  \ \text{subject to: }\quad G V_j = P_j \}
  \en
  which will yield the matrix of smallest F-norm satisfying the condition \nref{eq:msecant1}.
  Not surprisingly this matrix is just $G_{j+1}$.
  
  \begin{proposition}
  \label{prop:Boptim}
    The unique minimizer of Problem~\eqref{eq:optB} is the matrix $G_{j+1} $ given by
    \nref{eq:Gj}.
    \end{proposition}
    \begin{proof}
      The index $j$ is dropped from this proof. Exploiting orthogonal projectors
      we write $G$ as follows: $G = G V V^T + G (I - V V^T) = P V^T + G (I - V V^T)$ and observe that
      \begin{align*}
        \| G \|_F^2  &= \Tr [P V^T + G (I - V V^T) ] [ V P^T + (I - V V^T) G^T ] \\
        &= \Tr [P P^T]  + \Tr [G (I - V V^T)(I-VV^T)G^T  ] \\
                     & = \| P \|_F^2  + \| G (I - V V^T)\|_F^2 
      \end{align*}
      The right-hand side is minimized when $  G (I - V V^T) = 0$ which means  when
      $G = GV V^T$. Recalling the  constraint $G V = P$ yields the desired result.
      \end{proof} 

  

It is also possible to find a link between the method proposed herein
and the Anderson acceleration reviewed in Section~\ref{sec:AA1},
by unraveling  a relation with multi-secant methods.
%Note that equation~\nref{eq:msecant1} is satisfied for (at most) $m$ previous
%instances of $i$, i.e., at step $i$ we have 
%$ 
%  G_{j+1} v_i = p_i $ {for} $i=j_m, \cdots, j .  
%$ 
 % In other words we can also write
 Based on Proposition \ref{prop:Boptim}, we know that
\eq{eq:msecant1M}
 G_{j+1} V_j = P_j   .   
  \en  
  This is similar to the multi-secant condition
  $ G_j \mathcal{F}_j ={\cal X}_j $ of Equation
  \nref{eq:mscond} -- see also
  Equation (13) of \cite{FangSaad07} where   $  {\cal F}_j $
  and   $  {\cal X}_j $ are defined in \nref{eq:dfdx}.
  In addition, we also have a multi-secant version of the no-change
  condition \eqref{eq:msecant2}.
  This is similar to a block version of the no-change condition 
  Equation~\eqref{eq:NoCh} as represented by   Equation (15) of  \cite{FangSaad07},
  which stipulates that 
  \eq{eq:NoCh2} 
  (G_j - G_{j-m}) q = 0 \quad \forall q \perp \Span \{ \FF_j \} 
  \en
  provided we define  $ G_{j-m}= 0$. 
 
%%More links can be identified when setting $\beta = 0$ in Anderson acceleration.
Strong links can be established with the class of multi-secant methods to which AA belongs.
 Without loss of generality  and in an effort  to simplify notation we
also assume that $j_m = 1$ this time and $\beta=0$.
%% \textcolor{red}{YX: do we have to assume this?}
%% as stated: to simplify notation
 According to
 (\ref{eq:AA}--\ref{eq:thetaj}), the $j$-th iterate becomes simply
 $x_{j+1} = x_j - \XX_j \theta_j $ where
 $\theta_j$ is a vector that minimizes $\| f_j - \FF_j \theta \|$.
 For nlTGCR, we have $x_{j+1} = x_j + P_j y_j $
 where $y_j $ minimizes $ \| f(x_j) + V_j y \| $. So this  is identical with
 Equation \nref{eq:AA} when $\beta = 0$  in which  $P_j \equiv \XX_j$,
 and $\FF_j\equiv V_j$:

 \bigskip 
  \begin{center}
 \begin{tabular}{c|c c c c} \hline 
   AA     &   $\XX_j$ &   $\FF_j$   & $\theta_j$         \\  \hline
   nlTGCR &    $P_j$  &  $V_j$      & $- y_j$         \\ \hline
  \end{tabular}
  \end{center}

  \bigskip 
  In  multi-secant methods we set 
  \[ \FF_j = [f_1 - f_0, f_2 - f_1, \cdots, f_j - f_{j-1}] \quad
    \XX_j = [x_1 - x_0, x_2 - x_1, \cdots, x_j - x_{j-1}] \]
  and, with  $ G_{j-m} = 0 $,    the multi-secant matrix in \nref{eq:msec} becomes
  \eq{eq:AAb0}
    G_{j} = \XX_j  (\FF_j^T\FF_j)^{-1}\FF_j^T.
  \en 
  We restate the result from \cite{FangSaad07} that characterizes multi-secant methods also known
  as Generalized Broyden
  techniques~\cite{eyert:acceleration96}, for the particular case in which
$G_{j-m} \equiv 0$:  
  \begin{itemize}
  \item
    $G_j$ in \eqref{eq:AAb0} is the only matrix
    that satisfies both the secant condition \eqref{eq:mscond} and the no-change
      condition \eqref{eq:NoCh2};
    \item $G_j$ is also the matrix that minimizes $\| G \|_F $ subject to the condition $G \FF_j = \XX_j$.
      \end{itemize} 
   
    Consider now nlTGCR. If we set $\FF_j \equiv V_j $ and $\XX_j = P_j$ in Anderson,
    the multi-secant matrix $G_j$ in \nref{eq:AAb0} simplifies to \nref{eq:msecant1M} -
    which also minimizes $\|G \|_F$ under the secant condition
    $G V_j = P_j$.
    Therefore the two methods differ mainly in the way in which the sets
    $\FF_j / V_j$ ,  and $\XX_j / P_j $ are defined. Let us use the more general notation
    $V_j, P_j$ for the pair of subspaces. 

    In both cases, a vector $v_j$ is related to the corresponding $p_j$ by the fact that
    \eq{eq:ApproxNLT} v_j \approx J(x_j) p_j . \en
    In the case of nlTGCR this relation is explicitly enforced by
    a Frechet differentiation  (Line 10).     In the case of AA, we have  $v_j = \Delta f_{j-1} = f_j - f_{j-1} $ and the relation exploited
    is that
    \eq{eq:ApproxAA}
    f_j \approx f_{j-1} + J(x_{j-1}) (x_j - x_{j-1}) \to
      \Delta f_{j-1} \approx J(x_{j-1}) \Delta  x_{j-1}
      \en %-- before we perform an orthogonalization - which
    %combines this vector with others -- without changing the span of the new $P_j$ (and also
    %$V_j$). 



      
      However, relation \nref{eq:ApproxNLT} in nlTGMR is \emph{more accurate}
      because we use an additional function evaluation to explicitly obtain an
      accurate approximation (ideally exact value) for $J(x_j) p_j$. In
      contrast when $x_j$ and $x_{j-1}$ are not close, then \nref{eq:ApproxAA}
      can be a very rough approximation. This is a key difference between the
      two methods.
  
\iffalse  
 According to our earlier observation, $\XX_j$ is essentially the same as our $P_j$ - except for
 a scaling of the vectors. In addition, $\FF_j$ plays the role of our $V_j$ and
 what we call $y_j$ is the vector $\theta_j$ of AA. 
 If we had $\FF_j = V_j$ (up to scaling) the two methods would be identical.
 The only difference is the way in which the columns of $V_j$ are computed. It is important to note
 that 
\fi 




\iffalse

\subsection{Eigenvalue estimates as by-products}


We begin by reproducing the GCR algorithm for the linear case - in the situation when
$A$ is symmetric. In this case recall that the $\beta_{ij}$'s are all zero except
$\beta_{jj} $ which we now denote by $\beta_j$ (similar notation to CG)

We know that there is a strong relation between the Conjugate Gradient method and the
Lanczos vectors and this relation can provide eigenvalue estimates for the matrix $A$ in the
linear case -- see \cite[sec. 6.7.3]{Saad-book3}. It is also possible to derive a similar
result for the GCR algorithm. We wish to obtain a 3 term recurrence for building
an orthonormal basis of a Krylov subspace. Since the $A p_i$s are orthonormal it is natural to
consider these vectors.

As before we define  $v_j \equiv Ap_j$.
From Line~7 we get, upon multiplying through by $A$:
\eq{eq:Apj}
v_{j+1} = A r_{j+1} - \beta_j v_j
\en
But substituting the expresion of $r_{j+1}$ from Line~6 yields:
\eq{eq:Apj1}
v_{j+1} = A [r_j - \alpha_j v_j] - \beta_j v_j = = A r_j - \alpha_j A  v_j - \beta_j v_j .
\en
Next, from Line~7 used with $j$ instead of $j+1$ we have
$p_j = r_j - \beta_{j-1} p_{j-1}  \to
A r_j = v_j + \beta_{j-1} v_{j-1} $ and so we end up with:
\eq{eq:Apj2}
v_{j+1} = - \alpha_j A v_j + (1  - \beta_j)  v_j + \beta_{j-1} v_{j-1}
\en


  --------------------

  We rewrite the relation on the $v_i$s as
\[ 
  A v_j =  \frac{-1}{\alpha_j} v_{j+1}
  + \frac{1-\beta_j}{\alpha_j} v_{j}  + \frac{\beta_{j-1}}{\alpha_j} v_{j+1}   \]


This means that we have a tridiagonal representation of the matrix $A$ in the subspace
spanned by the $v_i$'s. This is identical with the Lanczos procedure.

--------------------

ALTERNATIVE PROJECTION METHODs. (1)
The above approach is not the only one if we want to estimate eigenvalues of $A$.
A second approach is to exploit the availabality of the bases $P$ and $AP$
and the fact that $AP$ is orthonormal.
We seek an approximate eigenpair
$\tilde \lambda, \tilde u$ where $\tilde  u  = P y$. Then writinf the Galerkin condition
\[
  (A - \tilde \lambda I) P y \perp \Span [A P]
\]
leads to 
\[
  (AP)^T (A - \tilde \lambda I) P y = 0
  \to [I - \tilde  \lambda P^T A P] y = 0
    \to [\frac{1}{\tilde  \lambda} I - P^T A P] y = 0 
\]
The advantage of the approaches discussed so far is that the matrices involved
are readily available and do not require any additional computations with
$A$. In the second case shown here we only need to compute inner products to get
$P^T A P$. 

ALTERNATIVE PROJECTION METHODs. (2)

We can also project only span(P) orthogonally to span(P)
Now we also seek an approximate eigenpair
$\tilde \lambda, \tilde u$ where $\tilde u = P y$ but the  Galerkin condition becomes
\[
  (A - \tilde \lambda I) P y \perp \Span [ P]
\]
which leads to a generalized eigenvalue problem 
\[
  (P)^T (A - \tilde \lambda I) P y = 0
  \to  P^T A P y =  \tilde \lambda  (P^T P ) y
\]


\fi


==> old_gcr.tex <==

\iffase 
\section{Nonlinear Truncated Generalized Conjugate Residual (nlTGCR) algorithm}\label{sec:linear} 
For understanding the conjugate residual-based methods in the nonlinear
case, it is important to first provide some background for
linear systems. A large
class of Krylov subspace methods for solving nonsymmetric linear systems have
been developed more than four decades ago. The reader is referred to the recent
volume by Meurant and Tebbens \cite{Meurant-Tebbens} which contains a rather
exhaustive and detailed coverage of these methods.
The main aim of the techniques proposed in
this article is to  adapt the residual-minimizing
subclass of Krylov methods for linear systems to the nonlinear case.
The guiding principle in this adaption is that we 
would like it to also approximately minimize the
nonlinear residuals. This is in contrast with inexact Newton methods
where the goal is to roughly solve the linear systems that arise in
Newton's method as a way to provide a good search direction.
%%We will argue that the common approach of \emph{Inexact Newton Methods}
%%utilized in the past leads to some weaknesses.

\subsection{The linear case:  Generalized Conjugate Residual (GCR) Algorithm}\label{sec:gcr} 
We first consider solving a linear system of the form:
   \eq{eq:Ax=b}  A x = b .
   \en
   Solving the above system is equivalent to
   finding the  minimum of the quadratic form 
   $\phi_q(x) \equiv \half \| b - A x\|_2^2 $.
   %% The goal is to solve
   %% $\nabla \phi_q = 0$, which leads to the linear system $Ax=b$.
Here, the gradient of $ \phi_q(x)$  is
$A^T (Ax-b)$ and its Hessian is the matrix $A^T A $.
However, standard methods based on this framework tend to be slow because
the condition number of $A^T A$ is usually large. As a result,
researchers developed methods based on using the standard residuals
$ r = b -A x$ to search for the minimum. 
Thus,  the  Generalized Conjugate Residual (GCR)
algorithm \cite{Eis-Elm-Sch} 
for solving \nref{eq:Ax=b} can formally be described as
shown in Alg. \ref{alg:gcr}.

%% 
    \begin{algorithm}[H]
    \centering
    \caption{GCR}\label{alg:gcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: Matrix $A$, RHS $b$,
  initial  $x_0$. \\
  Set $p_0=r_0 \equiv b-Ax_0$.
\For{$j=0,1,2,\cdots,$ until convergence} 
\State  $\alpha_j = (r_j, A p_j) / (A p_j, A p_j)$
\State $x_{j+1} = x_j + \alpha_j p_j$
\State $r_{j+1} = r_j - \alpha_j A p_j$
\State $p_{j+1} = r_{j+1} - \sum_{i=0}^j \beta_{ij} p_i $ \quad where \quad
$\beta_{ij} :=  (A r_{j+1} , Ap_i) / (A p_i, Ap_i)$
\EndFor
\end{algorithmic}
\end{algorithm}
The main point of the algorithm is to build a sequence of search
directions $p_i$, $i=1:j$ at step $j$ so that the vectors $A p_i$ are
orthogonal. This is done in Line~7.  With this we know that the
iterate as defined by Lines 4-5 is optimal in the sense that it yields
the smallest residual norm among solution vectors selected from the
Krylov subspace $x_0 + \mbox{span}\{p_0, \ldots, p_k\}$ -- see \cite[pp 195-196]{Saad-Book2}.  The GCR
algorithm is mathematically equivalent
\footnote{Here equivalent is meant in the sense that if exact arithmetic is
  used and if the compared algorithms both succeed in  producing the $j$-th
  iterate from the same initial $x_0$, then the two iterates are equal.} 
  from 
to GMRES~\cite{Saad-book3}, and
to some of the forms of other methods developed earlier, e.g.,
ORTHOMIN~\cite{Vinsome76}, ORTHODIR~\cite{Jea-Young}, and Axelsson's
CGLS method \cite{Axelsson80}.  
%A detailed account of Krylov subspace methods for nonsymmetric linear systems and their inter-relationships
%can be found in the exaustive treatise by Meurant and Duintjer
%Tebbens~\cite{Meurant-Tebbens}.

\iffalse
Eisenstat, Elman and Schultz established
a number of results including convergence for the situation when
$A$ is positive real, i.e., when the symmetric part of $A$ is positive
definite. Among other properties of the algorithm shown
are the orthogonality of the directions $Ap_i$, and the fact that
the iterate
$ x_{k+1}$ minimizes the residual norm over
$x_0 + \mbox{span}\{p_0, . . . , p_k\}$.
The orthogonality of the vectors $Ap_i$  is equivalent to the property that 
the directions $p_i$ are $A^TA$-orthogonal.
Another property of GCR  is that the 
residual vectors that it produces  are
`semi-conjugate' in that $ (r_i, Ar_j ) = 0$ for $i > j$.
\fi



\iffalse
the following theorem
- \cite{Eis-Elm-Sch}:
\begin{theorem}\label{thm:gcr}
  The following properties are satisfied by the vectors produced by
  Algorithm~\ref{alg:gcr}
\begin{enumerate}
\item $ (Ap_i, Ap_j ) = 0,$ for $ i \ne j$,
\item $ (r_i, Ap_j ) = 0,$ for $ i > j$,
\item $ (r_i, Ap_i  ) = (r_i, Ar_i )$,
\item $ (r_i, Ar_j ) = 0, i > j$,
\item $ (r_j , Ap_i ) = (r_0, Ap_i ), i \ge j$,
\item $ \{p_0, . . . , p_{k-1} \}$ and $\{r_0, . . . , r_{k-1} \} \
\mbox{span} \ K_k (A, r_0 )$, 
\item $ x_{k+1}$ minimizes the residual norm over $x_0 + \mbox{span}\{p_0, . . . , p_k\}$.
\end{enumerate}
\end{theorem}
\fi

Next we will discuss a truncated version of GCR
in which the $Ap_i$'s are only orthogonal to the $m$ previous
ones. This algorithm was first introduced by Vinsome as early as in 1976
and was named `ORTHOMIN' \cite{Vinsome76}. We will just refer to it as
the truncated version of GCR or TGCR.
%%Indeed it is unrealistic to keep all $A p_i$ vectors as this could require
%%an excessive amoumt of memory.
In what follows we will also write the algorithm in a form that is closer to a
practical implementation. Indeed, at step $j$ we need to keep a set of $m$ vectors
for the $p_i$'s and the other set for the vectors $v_i = A p_i$.  In addition, the orthogonalization in line~7 is a form of
classical Gram-Schmidt which we can replace by the modified form of Gram-Schmidt by
setting the vector $A r_{j+1} $ initially to a vector $v$ which is
orthogonalized against the successive $A p_i$s.  The resulting truncated GCR
algorithm is a slight variant of the original ORTHOMIN algorithm introduced 
in \cite{Vinsome76} and analyzed in  \cite{Eis-Elm-Sch}.
%%A number of methods were developed in the
%%1980s 1990s that were relatively close to each other, see \cite{Meurant-Tebbens}
%%for details.
  
\begin{algorithm}[H]
  \centering
  \caption{TGCR(m)}\label{alg:tgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: Matrix $A$, RHS $b$,
  initial  $x_0$. \\
  Set $r_0 \equiv b-Ax_0$; $v = A r_0$; 
  \State $v_0 = v/\| v \|$;   $p_0 = r_0 / \| v \|$; 
\For{$j=0,1,2,\cdots,$ Until convergence} 
\State  $\alpha_j = (r_j, v_j) $
\State $x_{j+1} = x_j + \alpha_j p_j$
\State $r_{j+1} = r_j - \alpha_j v_j$
\State $p = r_{j+1}$;  \quad  $ v = A p $;   \quad  and  \quad  $j_m = \max(0,j-m+1)$  
\For{$i=j_m:j$} 
\State $\beta_{ij} :=  (v, Ap_i) $
\State $p := p - \beta_{ij} p_i$;
\State  $v := v - \beta_{ij} v_i$; 
\EndFor
\State $p_{j+1} :=p /\| v\|$ ; \qquad  $v_{j+1} :=v/\|v\|$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}

As is seen in Line 3 and Line 14, we normalize each $v_i $ so $\| v_i \|=1$
and $p_i$ is normalized accordingly.
Steps 9--14 of the algorithm produce  a system of 
vectors 
$V_{j+1} = [v_{j_m}, v_{j_{m}+1},\ldots,v_j, v_{j+1}]$ that is orthonormal.
When $j \ge m$, $V_{j+1}$ consists of a `window' of $m+1$ vectors. Algorithm \ref{alg:tgcr} can be viewed as s method for approximately minimizing
the quadratic form $\phi_q(x) \equiv \half \| b - A x\|_2^2 $ in
a certain Krylov subspace.
With $m = \infty $ we obtain the non-restarted GCR method - which is equivalent to the non-started GMRES \cite{Saad-book3}.
The purpose of  Lines 8 to 14 is to compute the new direction $p_{j+1}$ --
by ortho-normalizing the vector $Ar_{j+1}$ against all previous $Ap_i$. From Line~11, we obtain
the relation $A p_{j+1} = A r_{j+1} - \sum_{i=j_m,j}  \beta_{ij}Ap_i$
from which it becomes clear that
$A p_{j+1} \perp A p_i $ for $i=j_m, \ldots,j$.

The properties in the next theorem were written in a slightly different form in
~\cite[Th. 4.1]{Eis-Elm-Sch}.
\begin{theorem}\label{thm:tgcr} 
  The following properties are satisfied by the vectors produced by
  Algorithm~\ref{alg:tgcr}
  \begin{enumerate}
\item  $(Ap_{j+1}, A p_i) = 0$, for $i = j_m,\ldots, j $ 
\item   $(r_{j+1}, Ap_i) = 0,$ for $ i=(j-1)_m,\ldots,j.$ 
\item  $(r_j, Ap_j) = (r_j, Ar_j)$,
\item  $(r_{j+1}, Ar_j) = 0$,
\item  $(r_j, Ap_i) = (r_{i-m}, Ap_i), j=i-m, \cdots,i, i \ge m$,
\item  if $r_i \ne 0$, then $p_i \ne 0$,
\item  for $i \ge m, x_{i+1}$ minimizes $\|b - Ax\|_2$ over the affine space
                              $x_{i-m} + \mbox{span} \{p_{i_m},\cdots p_i\}.$
\end{enumerate}
\end{theorem} 
                            
The same article \cite{Eis-Elm-Sch} establishes convergence of the algorithm
when $A$  is positive definite, i.e., when its
symmetric  part  is symmetric positive definite.
When $A$ is symmetric a number of simplifications
take place in Algorithm ~\ref{alg:gcr}.
In this  situation  it is known that the $\beta_{ij}$'s are all zero except
$\beta_{jj} $ which we now denote by $\beta_j$.
%%(in analogy with notation in CG). 
As a result
%%This leads to the  Conjugate Residual (CR)  algorithm  which is 
Algorithm~\ref{alg:gcr} simplifies:  Line 1-6 remain unchanged and
Line~7 is replaced by: 

\bigskip
\betab
\>7.cr:  \> \>
$p_{j+1} = r_{j+1} - \beta_{j} p_j $ \quad where \quad
$\beta_{j} :=  (A r_{j+1} , Ap_j) / (A p_j, Ap_j)$  .
\entab
\bigskip


%%\iffalse
The following alternative expressions for the scalars
$\alpha_j$ and $\beta_j$, that resemble those of the CG algorithm,
can be easily established 
%%by exploiting well-known properties of GCR:
\eq{eq:NewGCR}
\alpha_j = \frac{ (r_j, A r_j)}{ (A p_j, A p_j)} \qquad
\beta_j = - \frac{(A r_{j+1} , r_{j+1}) }{(A r_j, r_j) } . 
\en 
They yield the standard Conjugate Residual (CR)  algorithm
which dates back to Stiefel \cite{Stiefel-CR}, see
\cite[sec 6.8]{Saad-book3} for details.
\iffalse
These expressions are those used in the usual
  way of defining the Conjugate Residual (CR) algorithm 
  The CR Algorithm 
\fi
 
  \subsection{The nonlinear extention: nonlinear TGCR (nlTGCR) algorithm}\label{sec:nonlin}
  We now return to the nonlinear problem and ask the question:  how can we
  generalize the algorithms for linear systems of Section~\ref{sec:gcr} for solving nonlinear
  equations? We should begin by stating what are the desired features of this
  extension.
  First we would like the algorithms to  fall back to TGCR when the problem is linear.
  Second, we would like a method that can be adapted in such a way as to yield
  the inexact Newton viewpoint when desired or a multi-secant (AA-like) approach when
  desired. Third, we would like a method that exploits a more accurate linear model than
  either Newton or a quasi-Newton approach - possibly at the cost of  a few extra function
  evaluations. Finally, we would like the algorithm to be easily adaptable to the very
  common context in which the function $f$ is `fuzzy' as is the case when dealing with
  stochastic methods. 
  


\iffalse
  If there is no
  ambiguity we will denote $J(x_j)$ by $J$.  Note that the right-hand side of
  the Newton system is $-f(x_j)$ and this is also the residual for $x_j$, i.e.,
  when $\delta_j = 0$.
%  iterative refinement in the 
%  linear case where the right-hand side is the residual,
  Therefore, we will define the residual vector $r_j$  to  be $r_j = -f(x)$.
\fi 

  
  
  In our model we assume that at step $j$ we have a set 
  of (at most) $m$ current `search' directions
  $\{ p_i \} $ for $j_m \le i \le j$  gathered as columns of a matrix $P_j$,
  where we recall the notation $j_m \equiv \max\{0,j-m+1 \}$.
  Along with each $p_i$ we also assume that $v_i \equiv J(x_i) p_i $ is
  available and also   saved in a matrix denoted by $V_j$, so that
    \eq{eq:PjVj}
    P_j = [ p_{j_m}, p_{j_m+1},\cdots, p_j],
    \qquad 
    V_j = [ v_{j_m}, v_{j_m+1},\cdots, v_j].
    \en
    Note that this pair of matrices plays the same role as does the pair
    $\XX_j, \ \FF_j$ defined in \eqref{eq:dfdx} for Anderson acceleration.
  We then  write the linear model used locally as 
   \eq{eq:nltgcrmodle} f(x_j + P_j y) \approx f(x_j) + [J] P_j y \en where $[J] P_j$
  should be interpreted as \eq{eq:JP} [J] P_j \equiv [ J(x_{j_m})
  p_{j_m}, \cdots, J(x_{j}) p_{j} ] = V_j , \en
  i.e.,  the Jacobian  applied to each vector $p_i$ is calculated
  at the point $x_i$ and is therefore different for each $i$.
  While this is again somewhat similar to what was done for Anderson
  acceleration, we note a very important distinction that may have
  a siginificant effect on performance: \emph{In Anderson acceleration
    the linear model is simply based on the relation
    $f(x_j-\XX_j \theta) \approx f(x_j) -\FF_j\theta$ whereas nlTGCR evaluates
    explicitly  $J(x_i) p_i $.} This evaluation can be quite accurate if desired.
  In contrast, the relation
  $f(x_j-\XX_j \theta) \approx f(x_j) -\FF_j\theta$ can be quite rough,
  especially at the beginning of the process where the vectors $\Delta x_j$ and
 $\Delta f_j$ are not small.    
  
  The projection method will minimize the norm
  $\| f(x_j) + [J] P_j y \| = \| f(x_j) + V_j y \| $. This is achieved
  by determining $y$ in such a way that
  \eq{eq:opt} f(x_j) + V_j y \perp \Span \{V_j\} \
  \rightarrow \ (V_j)^T[f(x_j) + V_j y] = 0 \ \rightarrow \ y = 
  V_j^T r_j
  \en
  where it is assumed the the $v_i$'s are orthonormal.
  \iffalse Note that in the linear case, it can be shown that
  $v_i^T r_j = 0 $ for $j_m \le i < j$, so that $V_j^T r_j$ has only
  one nonzero component. The assumption that the $p_i$'s are fully
  orthogonal implies that $j_m$ is always equal to one.  In the
  situation we have partial orthogonality ($j_m > 1$) -- we can solve
  the least-squares problem explicitly instead of exploiting
  orthogonality.  A simpler alternative is just to redefine $P_j$ and
  $V_j$ to consist of their columns $j_m $ to $j$ which are
  orthogonal.
\fi 
    
  
Instead  of (\ref{eq:inex1}--\ref{eq:inex2}) of the inexact Newton approach
we now have an iteration of the form
    \begin{align} 
 &      \mbox{Find}  & y &= \mbox{argmin}_y \| f(x_j) + V_j y \|  &  \label {eq:inex3}\\
 &       \mbox{Set}  & x_{j+1}  & = x_j + P_j y_j & \label {eq:inex4}
  \end{align}  
  A major distinction between this approach and standard inexact
  Newton is that the latter exploits approximations to the Jacobian
  around one point in order to build the next iterate.  The iterates
  generated by the iterative process can be viewed as intermediate
  points but they rely on an a Jacobian calculated $J(x_0)$ at the initial
  approximation.
  %%Thus, intermediate iterates do not use updated
  %%versions of the Jacobian.
  We will revisit the inexact Newton viewpoint in a  later   section.

  \iffalse 
  The proposed approach uses $m$ pairs of vectors $p_i, J(x_i) p_i$.
  %% and as was already mentioned
 these pairs resemble the pairs $\Delta x_j, \Delta f_j$ of AA.
 However, in our case, computing $J(x_i) p_i$  comes at the cost of
 doubling the number of function evaluations,
 although  the local model is likely to be more accurate and this could be
 more important at the beginning of the process. 
 \fi
 
   The idea of the nonlinear version of the truncated GCR method is to
   exploit the directions that are produced by the TGCR algorithm.
   Note here is that there is a decoupling between the \emph{update}
   from the current iterate to a new one (lines 5--6) and the
   \emph{construction of the $p_i$'s} in TGCR (lines 8--14).  In
   essence, the first part just builds a new approximation given a new
   `search' subspace - while the second adds a new direction to this
   evolving subspace, by exploting the most recemt residual (line
   8).
   This distinction will help us generalize our approach to cases where
   the objective function or the Jacobien varies as the iteration proceeds.
   
   %% In the nonlinear case, we must take this residual to be the   nonlinear one.

    \begin{algorithm}[htb]
    \centering
    \caption{nlTGCR(m)}\label{alg:nltgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: $f(x)$,   initial  $x_0$. \\
  Set $r_0 = - f(x_0)$.
  \State Compute  $v = J(x_0)  r_0$; \ (Use Frechet)
  \State $v_0 = v/ \| v \| $, $p_0 = r_0/ \| v \| $;
  \For{$j=0,1,2,\cdots,$ } 
\State  $y_j = V_j^T r_j $ 
\State $x_{j+1} = x_j + P_j y_j$
\State $r_{j+1} = -f(x_{j+1}) $ 
\State Set: $p := r_{j+1}$; and $j_m = \max(0,j-m+1)$
\State Compute $v =  J(x_{j+1})  p$ (Use Frechet)
\For{$i=j_m:j$}
\State $\beta_{ij} :=  (v, v_i) $
\State $p := p - \beta_{ij} p_i$
\State $v := v - \beta_{ij} v_i$
\EndFor
\State $p_{j+1} :=p /\| v\|$ ; \qquad  $v_{j+1} :=v/\|v\|$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}


  
  We now derive our general algorithm from which a few variants will follow.
  The algorithm is an extension of Algorithm~\ref{alg:tgcr} -- with a few
  needed changes that reflect the nonlinearity of the problem.
  The first change is that any residual is now to be replaced by the negative of
  $f(x)$ so  Line~2 of Algorithm~\ref{alg:tgcr} becomes
  $r_0 = -  f(x_0)$ and Line~7 must be replaced by
  $r_{j+1}  = -  f(x_{j+1})$. In  addition, the matrix $A$ in   the 
  products  $A  r_0  $  and  $A  p$ invoked  in    Line~2  and  Line~8
  respectively, is the   Jacobian of  $f$ at the most recent 
  iterate.  The most
  important  change is  in  lines  6-7 where  according  to the  above
  discussion the scalar $\alpha_j$  of Algorithm~\ref{alg:tgcr} is to be replaced
  by the 
  vector $y_j$ that  minimized $\| f(x_j) + V_j y \|$ over $y$.
  The reason for this was explained above.  
%%    $(v_j ,v_i) = \delta_{ij} \quad \mbox{for}\quad j_m \le i \le j $

  
The resulting algorithm is shown in Algorithm~\ref{alg:nltgcr}.  
It requires two function evaluations per step : one in Line 8 and the
other in Line~10.  In the situation when computing the Jacobian is
inexpensive, then one can compute $J p$ in Line~10 as a matrix-vector
product. Apparently, the system $[v_{j_m}, v_{j_m +1}, \cdots,  v_{j+1}] $ is orthonormal. 
%and this will reduce the number of function evaluations per step from 2 to 1.
%% Next we examine properties ..

  
\section{Theoretical results}
In this section, we analyze the connections of the nlTGCR algorithm to inexact Newton and quasi-Newton methods as well as its convergence results.
\subsection{Linearized update version and the connections to inexact Newton methods} 
In this section, we first consider a variant of the algorithm which we call
the ``linearized update version''. We will show that this version is equivalent to inexact Newton methods in which the system is approximately solved with TGCR. Two changes are made to Algorithm \ref{alg:nltgcr} to obtain this linearized update version. 
First,  in Line~8 we update the
residual by using the linear model, namely, we replace Line~8 by: 
 
\bigskip
%%\hrule
\betab
\> 8a:  \> \>  $ r_{j+1} = r_j - V_j y_j$
\entab
\smallskip 


%% In addition, in order to obtain the exact equivalent of
%% inexact Newton methods,

The second change is that the Jacobian is not updated in Line~10, i.e.,
$J(x_{j+1})$ in Line 10 is kept constant
and equal to $J(x_0)$. In other words
$v$ is computed as
\bigskip
\betab
\> 10a:  \> \>   $ v = J(x_0) p $ 
\entab
\smallskip 

%%If $k$ steps of the algorithm are carried out we would get what amounts to
%%When $F$ is linear, then the residual at step $j+1$ becomes
%%$r_{j+1} = b - A(x_j + P_j y_j) = r_j - A P_j y_j $ and we recall that
%%$Ap_i$ is saved as $v_i$.
%% In addition, in order to obtain the exact equivalent of
%% inexact Newton methods, the Jacobian $J$ in Line 10 is kept constant
%% and equal to $J(x_0)$.

The algorithm is stopped  when the residual norm $r_{j+1} $
is small enough or the number of steps is exceeded.
In addition, \emph{we consider the algorithm merely as a means of providing
  a search direction} as is often done with inexact Newton methods.
In other words the direction $d = x_{last} - x_0$ is provided
to another function which will use it in an iteratire procedure
which will include a linesearch technique at $x_0$. 

It is easy to see that one iteration defined as a sweep using
$k$ substeps of this   linear update version is nothing but
\emph{an inexact Newton method in which the system \nref{eq:inex1}
  (with $j=0$) is approximately solved with the TGCR algorithm.}
Indeed, in this situation Lines 4-15 of Algorithm~\ref{alg:tgcr} and Lines
5-17 of Algorithm~\ref{alg:nltgcr} are identical.
Lines 5-17 of Algorithm~\ref{alg:nltgcr}  perform $k$ steps of
the TGCR algorithm to  solve the linear systems $f(x_0) + J(x_0) P y = 0$.
Within Algorithm~\ref{alg:nltgcr}  the update is written in progressive form
as $x_{j+1} = x_j + \alpha_j p_j$, note that
\emph{the right-hand side does
not change during the algorithm and is equal to $r_0 = - f(x_0)$.
}
In effect the last  iterate - $x_k$ is updated from $x_0$ by adding a vector from the Krylov subspace
or equivalently the span of $P_k$.
As a consequence of this observation, 
it turns out that $y_j$ has only one nonzero
component,  namely the last one. 
Indeed, from part 2 of Theorem \ref{thm:tgcr} we see that if we replace
$A$ by the Jacobian $J$ at $x_0$ then:
\[
  (r_{j+1}, J p_i) = 0  \ \mbox{for} \ i=(j-1)_m, \cdots, j. 
\]

It was shown in \cite{Brown-Saad} that under mild conditions, the update to the
iterate is a descent direction. In addition, the article describes `global
convergence strategies' based on linesearch and trust-region techniques.  If we
do not apply a global convergence strategy, then the algorithm may have difficulties
to converge.


{Inexact Newton methods \cite{Dembo-al} 
are often implemented with residual reduction stopping criteria of the form
\eq{eq:forcing}
\| f(x_j) + J(x_j) \delta_j \| \le \eta_j \| f(x_j) \|
\en
where  $\eta_j \in [0,1) $ is called the forcing term.
This only means that the iterative procedure that is applied when
approximately solving the linear system \nref{eq:inex1} exits when
the relative residual norm falls below $\eta_j$.
In this context, the following assumptions on $f$ are made
\cite{Dembo-al}: 
\begin{itemize}
  \item  There exists a $x_* \ \in \ \RR^n$  with $f(x_*)= 0$.
  \item $f$ is $C^1$  in a neighborhood of $x_*$.
  \item $J(x_*) = f’(x_*)$  is nonsingular.
  \end{itemize}
  Under these conditions and assuming that the forcing term is such that
  $\eta_j  \le  t < 1$ then Dembo et al \cite{Dembo-al} prove a local convergence result: there is an
  $\epsilon$ such if $ \| x_0 - x_*\| \le \epsilon$ then $x_j$ will converge to $x_*$.
  In addition the convergence is linear. Superlinear convergence can be achieved by
  requiring that $\eta_j \to 0$.}


As was already mentioned, inexact Newton methods have a number of
disadvantages.  Probably the most significant is that a large
number of function evaluations may be needed to build the Krylov
subspace in order to obtain a single iterate, i.e., the  next  iterate. 
After this iterate is computed, all the information gathered at
this step, e.g., $P_k, V_k$, is discarded. This is to be contrasted with
a method like Quasi-Newton where the most recent function evaluation
contributes to building an updated approximate Jacobian.

\subsection{Nonlinear update version}
The ``linearized update version" of Algorithm~\ref{alg:nltgcr} discussed above uses
a simple linear model to update the residual $r_j$ in which the Jacobian is not updated.
Next, we consider the ``nonlinear update version" as described in
Algorithm~\ref{alg:nltgcr}. %This version explicitly enforces the linear
%optimality condition of GCR, as represented by Equation~\nref{eq:opt}.

Assume a sweep using
$j$ substeps of Algorithm~\ref{alg:nltgcr} has been carried out. Our next result will invoke the  linear residual
\eq{eq:LinRes} \tilde r_{j+1} = r_j - V_j y_j , \en
as well as the deviation between the actual residual $r_{j+1}$ and its
linear version $\tilde r_{j+1}$ at the $j+1$th iteration: 
\eq{eq:ResDev} z_{j+1} = \tilde r_{j+1} - r_{j+1} . \en 

 
We first analyze the magnitude of $z_{j+1}$. Define
\eq{eq:wi}
w_i = (J(x_j) - J(x_i)) p_i \ \mbox{for} \ i=j_m, \cdots, j ;  \quad \mbox{and}\quad 
W_j = [w_{j_m}, \cdots, w_j ].
\en
%% ---- delta_j --> s_j
Observe  that
\eq{eq:Jxjpi}
  J(x_j) p_i = J(x_i) p_i + w_i = v_i + w_i .
  \en
  We also define:
\eq{eq:2ndOrd}
s_j  = f(x_{j+1}) - f(x_j) -  J(x_j) (x_{j+1} - x_j) . 
\en
Recall  from the Taylor series expansion $s_j$ is a second order term relative
to $\| x_{j+1}-x_j \|_2$. 
Then we derive the following bound on the norm of $z_{j+1}$ in the next proposition.


\begin{proposition}\label{prop:2}
  The difference $\tilde r_{j+1} - r_{j+1} $ satifies the relation:
\eq{eq:ResDiff}
\tilde r_{j+1} - r_{j+1}  =   W_j y_j  + s_j
=   W_j V_j^T r_j  + s_j ,
\en
and therefore:
\eq{eq:ResDiffN}
\| \tilde r_{j+1} - r_{j+1} \|   \le \| W_j \|_2  \ \| r_j \|_2 + \| s_j \|_2 . 
\en

\end{proposition}

\begin{proof} 
We rewrite the difference as:
\begin{align}
  \tilde r_{j+1} -r_{j+1}
  & = (-f(x_j) - V_j y_j ) + f(x_{j+1})  \nonumber\\
  & = (f(x_{j+1}) - f(x_j))  - V_j y_j  \nonumber\\
  & = J(x_j) P_j y_j + s_j - V_j y_j \label{eq:prop2pf}
\end{align}       

Letting $ y_j = [ \eta_1, \eta_2, \cdots ]$ we  get
\begin{align}
  J(x_j) P_j y_j
  &= \sum  \eta_i J(x_j) p_i  \nonumber \\
  &= \sum \eta_i J(x_i) p_i   + \sum \eta_i (J(x_j) -J(x_i)) p_i \nonumber\\
  &= V_j y_j  + W_j y_j . \label{eq:prop2pf2} 
  \end{align}
The proof follows by combining \eqref{eq:prop2pf2} and \eqref{eq:prop2pf}.
\end{proof}
 
The proposition shows that $z_{j+1}$ is a quantity of the second order:
$\| W_j \|_2 \| r_j \|_2 $ is the product of \textcolor{blue}{2 first order terms} \textcolor{red}{YX: is $r$ a first order term? Why?} while $s_j$ is a second
order term according to its  definition \nref{eq:2ndOrd}. Let us explore this a little further by making the assumption that:
 \eq{eq:2ndOrd1}
 \| (J(y) - J(x)) p  \| \le   L_h \|x-y\|  \ \| J(x) p \| . 
 \en
 Recalling that $\|J(x_i)  p_i \| = \|v_i \| = 1$, we get

 \eq{eq:wibnd} 
   \|w_i \| = \| (J(x_j) - J(x_i)) p_i\| \le
   L_h \| x_j - x_i \| \| J(x_i)  p_i \| =       L_h \| x_j - x_i \|
   \en
      and it follows from \nref{eq:wibnd} that
  \[
   \| W_j\|_2 \| r_j \| \le  m_j L_h \times \frac{1}{m_j} \sum \|x_i - x_j \|  \ \| r_j \| \]
  The term
 \[  \frac{1}{m_j} \sum \|x_i - x_j \|  \equiv \rho_j \]
 denotes the average distance from the previous $j_m$ iterates
 $x_i $ to $x_j$. Thus, we have 
 \eq{eq:bndWr}
 \|W\|_2 \| r_j \|_2 \le m_j L_h \rho_j \|r_j\| .
 \en
 When the process is nearing convergence, the right-hand side is clearly
 \textcolor{blue}{a second-order term}. Furthermore, we can prove the following properties of Algorithm~\ref{alg:nltgcr}.
\begin{proposition}\label{prop:nltgcr} 
    The following properties are satisfied by the vectors produced by
    Algorithm~\ref{alg:nltgcr}:
    %% where $e_{1,k} $ is the $1$st column of the identity matrix    of dimension $k$.
    

  \begin{enumerate}
 

  \item 
    $ ( \tilde r_{j+1}, v_i) = 0  \quad \mbox{for} \quad j_m \le i \le j$,
    i.e., $V_{j}^T \tilde r_{j+1} = 0$.

    
  \item 
    $ \| \tilde r_{j+1} \|_2 = \min_y \| -f(x_j) + [J] P_j y\|_2
    = \min_y \| -f(x_j) + V_j y\|_2 $

    
  \item $(v_{j+1} , \tilde r_{j+1})
    = \left( v_{j+1} \ , r_j \right) $

  \item $y_j=V_{j}^T r_{j} = (v_{j}, \tilde r_{j}) e_{m_j} - V_{j}^T z_{j}  $
    where $ e_{m_j} = [0, 0, \cdots, 1]^T \in \ \RR^{m_j}$ with $m_j \equiv \min \{m, j+1\}$.
    
%%  \item $V_{j}^T r_{j} = (v_{j}, \tilde r_{j}) e_{1,m_j} + V_{j}^T z_{j}  $
%%    where $ e_{1,m_j} = [1, 0, \cdots, 0]^T \in \ \RR^{m_j}$ with $m_j = \min \{m, j+1\}$.

\end{enumerate}

\medskip 
\end{proposition}

\begin{proof} 
  Properties (1) and (2) follow from the definition of the algorithm.
  For Property (3)  first observe  that
  $V_j = [v_{j_m}, v_{j_m+1},\cdots, v_{j-1}, v_j]$
  and that $v_{j+1}$ is made orthogonal against  the $m_j$ vectors    $v_{j_m}$ to $ v_j$,
  so $ v_{j+1}^T  V_j  = 0 $ and
  \[
  v_{j+1}^T  \tilde r_{j+1}   =  v_{j+1}^T [r_j - V_j y_j]
  \ = \   v_{j+1}^T r_j . 
  \]

  It is convenient to prove  Property (4)  for the index $j+1$. We write:
  $     V_{j+1}^T r_{j+1} =  V_{j+1}^T [\tilde r_{j+1} - z_{j+1} ] $ 
where $z_{j+1} $ was defined in Equation \eqref{eq:ResDev}.
  Recalling Property (2), we have that
  $(\tilde r_{j+1}, v_i ) = 0 $ for $j_m \le i \le j$ - so there is only one nonzero term
  in the product $V_{j+1}^T \tilde r_{j+1}$, namely  $v_{j+1}^T \tilde r_{j+1}$, i.e.,
  \[   \tilde r_{j+1}^T V_{j+1}
  = \tilde r_{j+1}^T [v_{(j+1)_m}, \cdots,  v_j, v_{j+1} ]
  = [0, 0 , \cdots, 0,   \tilde r_{j+1}^T v_{j+1} ]
  = \tilde r_{j+1}^T v_{j+1} e_{k}^T 
\]
where $e_k \ \in \ \RR^k$ and
$k$ is the number of columns in $V_{j+1}$, which is $\min \{m, j+2\}$
(recall: indexing starts at $j=0$ so $V_{j+1}$ has $j+2$ columns when $j+2\le m$).
This gives the results after adjusting for the change of index.
\end{proof}   

Property (4) and Proposition \ref{prop:nltgcr} indicate that when $z_j$ is small, as when the model \emph{close to being linear} \textcolor{blue}{YX: or near convergence},
then  $y_{j} $ will have small components everywhere except for the last component. 
As a result we may consider a variant of the algorithm
whereby $y_j$ is truncated so as to contain only its \textcolor{blue}{last entry}. \textcolor{blue}{This variant will be
studied in Section~\ref{sec:nlSimpl}.} \textcolor{red}{YX: Do we need to keep this option as we haven't implemented this in our code.}

\textcolor{red}{YX: When we switch from nonlinear update to linear update, we check $\Vert z_j\Vert_2$ explicitly in our implementation. Can we check the first $m_j-1$ entries in $y_j$ instead?}


 \subsection{Update vectors as  descent directions} 

Next we want to study under what conditions,  the update vector
is a descent direction. Here we call update vector the vector 
$d_j = P_j y_j$ with $y_j = V_j^T r_j$, which updates $x_j$ into
$x_{j+1} = x_j + d_j$, see in Lines 6-7 of Algorithm~\ref{alg:nltgcr}. 



DO NOT REMOVE 

There are a number of choices we can make for an objective function $g(x)$ if we are
to examine whether or not $d_j$ is a descent direction for this function. A common approach used when solving nonlinear systems of equations,
is to examine whether or not $d_j$ is a descent direction for the function
%%We would like to see if $d_j$ is a
%%descent direction for an appropriate function $f$. 
%% Question: is the vector $d_j=P_j y_j$ a descent direction for
$g(x) = (1/2) \| f(x) \|^2_2$. For this case,  recall that
$\nabla g(x) = J(x)^T f(x) $.
We now consider the inner product:
  \eq{eq:PrfDesc0} 
  (\nabla g(x_j), d_j)
  = (J(x_j)^T f(x_j), P_j V_j^T r_j)= - (J(x_j)^T r_j, P_j V_j^T r_j)  .
  \en


  A few algebraic manipulations lead to the following proposition.

  

  \
  \begin{proposition}\label{prop:3}
    Let $g(x) = \half \| f(x)\|_2^2 $ and let
$\tilde v_{j_m}, \cdots, \tilde v_j$ be the columns of:
\eq{eq:tilV}
\tilde V_j \equiv J(x_j) P_j . \
\en 
Then, 
  \eq{eq:prop3} 
  (\nabla g(x_j), d_j)
  = - (v_{j}, r_j)^2 -  \sum_{i=j_m}^{j-1} (v_i, r_j) ( \tilde v_{i}, r_{j}).
  \en
\end{proposition}
\begin{proof} 
%%%    & \equiv - ( \tilde V_j^T r_j, V_j^T r_j) \label{eq:delbyd}. 
  From  Property~(4) of Proposition~\ref{prop:nltgcr} we have
  $  V_j^T r_j = (v_{j}, \tilde r_{j}) e_{m_j} -  V_{j}^T z_{j} $ and so
  \begin{align*} 
  (\nabla g(x_j), d_j)
  &= - (J(x_j)^T r_j, P_j [ (v_{j}, \tilde r_{j}) e_{m_j} -  V_{j}^T z_{j} ]) \\
    & = - (v_{j}, \tilde r_{j}) (J(x_j)^T r_j, p_j) + (J(x_j)^T r_j, P_jV_{j}^T z_{j})\\
    & = - (v_{j}, \tilde r_{j}) (r_j, J(x_j) p_j) + (r_j,  J(x_j) P_j V_{j}^T z_{j} ) \\
    & = - (v_{j}, \tilde r_{j})(v_{j}, r_{j})  + (r_j, \tilde V_j V_{j}^T z_{j})\\
    & = - (v_{j}, r_j + z_j)(v_{j}, r_{j})      + (r_j, \tilde V_j V_{j}^T z_{j} ) \\
    & = - (v_{j}, r_j)^2 -  (v_{j}, z_j)(v_{j}, r_{j}) + (r_j, \tilde V_j V_{j}^T z_{j} ) .
   \label{eq:PrfDesc1} 
  \end{align*} 
  We write the middle term in the final expression as
  $(v_{j}, z_j)(v_{j}, r_{j}) = (r_j, (v_j v_j^T) z_j)$ and the product
  $\tilde V_j V_j^T z_j$ in the form $\tilde V_j V_j ^Tz_j  = \sum_{i=j_m}^j \tilde v_i v_i^T z_j$. 
  Next, we note that the last column of
  $\tilde V_j$ is equal to $J(x_j) p_j $ which is $v_j$.
  The result is that the product
  $ (r_j, (v_j v_j^T) z_j)$ cancels the last term 
  in the sum (the term corresponding to $i \equiv j$ in the summation) and we end up with
  \eq{eq:PrfDesc2} 
  (\nabla g(x_j), d_j)
     = - (v_{j}, r_j)^2 +  \sum_{i=j_m}^{j-1} (r_j, \tilde v_i v_{i}^T z_{j}).
     \en
     Next observe that for each of the terms in the sum we have:
     \[
       v_{i}^T z_{j} = v_{i}^T (\tilde r_j - r_j) = -v_{i}^T r_j
     \] 
     since $\tilde r_{j} \perp V_{j-1}$.  This gives
  \eq{eq:PrfDesc3} 
  (\nabla g(x_j), d_j)
  = - (v_{j}, r_j)^2 -  \sum_{i=j_m}^{j-1} (r_j, \tilde v_i v_{i}^T r_{j})
  = - (v_{j}, r_j)^2 -  \sum_{i=j_m}^{j-1} (v_i, r_j) ( \tilde v_{i}, r_{j}).
     \en
\end{proof}

We have  $v_i = J(x_i) p_i$ while $\tilde v_i  = J(x_j) p_i$.
Near convergence, the two vectors will be close enough that the
inner products
$(v_i, r_j)$ and $ ( \tilde v_{i}, r_j)$ will have the same sign in which case
the inner product \nref{eq:prop3} is negative and $d_j$ is a descent
direction.
In addition, we saw in the proof that $(v_i, r_j)= -(v_i, z_j)$ for $j_m \le i \le j-1$.
Thus, the terms $(v_i, r_j) ( \tilde v_{i}, r_{j})$ are likely smaller order terms.

\iffalse
An interesting property links the matrices  $V_j$ and $\tilde V_j$.
Let us denote by $\beta_{j+1,j} $ the scalar $ \| v \|_2$ used in the normalization
step of Algorithm~\ref{alg:nltgcr}, in Line 16. Then the following Arnoldi-like
relations can be extracted from the algorithm
\begin{align}
  r_{j+1}             &= \sum_{i=j_m}^{j+1} \beta_{ij} p_i \label{eq:piHess} \\
 J(x_{j+1})   r_{j+1} &= \sum_{i=j_m}^{j+1} \beta_{ij} v_i \label{eq:viHess}
\end{align}
Denoting by $b_j $ the vector of components $\beta_{ij}$ and multiplying
\nref{eq:piHess} by $ J(x_{j+1}) $ we obtain
\[
  \tilde V_j b_j = V_j b_j =  J(x_{j+1}) r_{j+1} .  
  \]
\fi
\textcolor{red}{YX: if $d_j$ is not a descent direction, we can simply choose $-d_j$. If this is the case, why do we need the simplied nonlinear update algorithm discussed in the next subsection}

\textcolor{red}{YX: should we add the convergence result with line search? We only show that the update direction is always a descent direction.}

\textcolor{red}{YX: when Jacobian is indefinite, we found nltgcr is not numerically equivalent to GMRES. Moreover, nltgcr does not provide a descent direction (as seen in LJ experiment).}

\textcolor{red}{YX: The descent direction check implemented in the code is different from the discussion here. We ignore the Jacobian in the computation of the inner product in the implementation.}
\subsection{Simplified nonlinear update algorithm} \label{sec:nlSimpl}
\textcolor{red}{YX: do we need this subsection as we haven't implemented this in the code?}

We can derive a simplified version of the algorithm
in which Lines 6 and 7 are replaced by Lines 5 and 6
of Algorithm~\ref{alg:tgcr} for linear systems,  i.e,
\eq{eq:nltgcr2}
\alpha_j = (r_j, v_j) \qquad x_{j+1} = x_j + \alpha_j p_j
\en

Often in practice there is little difference between the two because the vector $y_j$ is
often dominated by  $\alpha_j$. 
In this regard, 
we have the following useful property.

\begin{proposition}
  Assume that at step $j$ we have $\alpha_j \ne 0$, i.e., $(v_j, r_j) \ne 0$.
  Then the direction $d = \alpha_j p_j$ is a descent direction for the
  objective function $g(x) \equiv \half \Vert f(x)\Vert_2^2$.
\end{proposition}
\begin{proof}
  The gradient of $g(x_j) $ is $ J(x_j)^T f(x_j)$
  and so $d$ is a descent direction if
  $  (J(x_j)^T f(x_j), d ) <0 $.
  Next, recall that $r_j = - f(x_j) $ and so
  \[  (J(x_j)^T f(x_j), \alpha_j p_j ) = ( f(x_j), \alpha_j J(x_j) p_j )
    =  \alpha_j ( f(x_j),  v_j ) = -\alpha_j^2 < 0 .
    \] 
  \end{proof}

\textcolor{red}{YX: should we expand the following statement. Or if one direction leads to descent direction, can we show that using $V^Tr_j$ is better than this?}
  This means in particular that a linesearch backtracking strategy can be applied with all the
  related results on global convergence.
  
\textcolor{blue}{
  Next we examine properties similar to those established in \cite{Eis-Elm-Sch} for TGCR.
  First define the \emph{linear residual} at step $j$ as
  \eq{eq:linRes}
  \hat r_{j+1} = -f(x_j)-\alpha_j v_j .
  \en
  The idea is that we are solving a linear system approximately by a
  descent type method and the residual shown above is 
  residual corresponding to this solve.
  Property: $ \| \hat r_{j+1} \|_2^2 = \| r_{j} \|_2^2 - \alpha_j^2 $
  proof: $ \hat r_{j+1} \perp v_j $
  Property:
  \[ (\hat r_{j+1}, v_i ) = (r_{j}, v_i )  \quad
    \mbox{for} \quad \ j-m+1 \le i \le j \]
  %%%% 
  In what follows
  we assume that each $J(x_i) p_i$ is evaluated exactly and that
  $m = \infty$.}
  
\textcolor{red}{YX: Line search implementation is missing and switch from nonlinear update to linear update version and vise verse. Should we check $z_j$ directly or check $y_j$?}

%%  Here again we see that the inner product is dominated by the
%%  term $-(v_j, r_j)^2 $ and the rest is a second order term.
  
 
 \subsection{Connections to quasi-Newton and multiscent methods} 
In this section, we show that nlTGCR can be viewed from the alternative angle of
a quasi-Newton/multisecent approach. In this viewpoint,  the inverse of the Jacobian
is approximated progressively. Because it is the inverse Jacobian that is
approximated, the method is akin to Broyden's second update method.

First  observe that in nlTGCR  the update at step $j$ takes the form:

\[x_{j+1} = x_j + P_j V_j^T r_j = x_j + P_j V_j^T (-f(x_j)) . \]
Thus, we are in effect using a secant-type method.
The approximate inverse Jacobian at step
$j$, which we denote by  $G_{j+1} $ for consistency with common
notation, is equal to
\eq{eq:Gj}
G_{j+1} = P_j V_j^T .
\en 
If we apply this to $v_i$ we get
$
  G_{j+1} v_i = P_j V_j^T v_i =  p_i =  J(x_i) \inv v_i \quad \mbox{for} \quad j_m \le i \le j.
$ 
So $G_{j+1}$ inverts $J(x_i)$ exactly when applied to $v_i$. It therefore satisfies 
the \emph{secant} equation
\eq{eq:msecant1} 
  G_{j+1} v_i = p_i \quad \mbox{for} \quad j_m \le i \le j,
  \en
which is a version of \nref{eq:secant2}   used in    Broyden's second update method.
Here,  $p_{i}$ plays the role of $\Delta x_j$ and $v_i$ the role
  of $\Delta f_j$.
In addition, the update $G_{j+1}$ satisfies the `no-change' condition:
\eq{eq:msecant2} 
  G_{j+1} q = 0 \quad \forall q \perp v_i  \quad \mbox{for} \quad j_m \le i \le j.
  \en
  The usual no-change condition for secant methods is of the form
  $(G_{j+1}-G_{j-m}) q = 0 $ for $q \perp \Delta f_i$ which in our case
  would be
  $(G_{j+1}-G_{j-m}) q = 0 $ for $q \perp \ v_i  \quad \mbox{for} \quad j_m \le i \le j$.
  One can  therefore consider that we are updating $G_{j-m} \equiv 0$.




  Thus, consider the optimization problem
  \eq{eq:optB}
  \min \{  \| G \|_F  \ \text{subject to: }\quad G V_j = P_j \}
  \en
  which will yield the matrix of smallest F-norm satisfying the condition \nref{eq:msecant1}.
  Not surprisingly this matrix is just $G_{j+1}$.
  
  \begin{proposition}
  \label{prop:Boptim}
    The unique minimizer of Problem~\eqref{eq:optB} is the matrix $G_{j+1} $ given by
    \nref{eq:Gj}.
    \end{proposition}
    \begin{proof}
      The index $j$ is dropped from this proof. Exploiting orthogonal projectors
      we write $G$ as follows: $G = G V V^T + G (I - V V^T) = P V^T + G (I - V V^T)$ and observe that
      \begin{align*}
        \| G \|_F^2  &= \Tr [P V^T + G (I - V V^T) ] [ V P^T + (I - V V^T) G^T ] \\
        &= \Tr [P P^T]  + \Tr [G (I - V V^T)(I-VV^T)G^T  ] \\
                     & = \| P \|_F^2  + \| G (I - V V^T)\|_F^2 
      \end{align*}
      The right-hand side is minimized when $  G (I - V V^T) = 0$ which means  when
      $G = GV V^T$. Recalling the  constraint $G V = P$ yields the desired result.
      \end{proof} 

  

It is also possible to find a link between the method proposed herein
and the Anderson acceleration reviewed in Section~\ref{sec:AA1},
by unraveling  a relation with multi-secant methods.
%Note that equation~\nref{eq:msecant1} is satisfied for (at most) $m$ previous
%instances of $i$, i.e., at step $i$ we have 
%$ 
%  G_{j+1} v_i = p_i $ {for} $i=j_m, \cdots, j .  
%$ 
 % In other words we can also write
 Based on Proposition \ref{prop:Boptim}, we know that
\eq{eq:msecant1M}
 G_{j+1} V_j = P_j   .   
  \en  
  This is similar to the multi-secant condition
  $ G_j \mathcal{F}_j ={\cal X}_j $ of Equation
  \nref{eq:mscond} -- see also
  equation (13) of \cite{FangSaad07} where   $  {\cal F}_j $
  and   $  {\cal X}_j $ are defined in \nref{eq:dfdx}.
  In addition, we also have a multi-secant version of the no-change
  condition \eqref{eq:msecant2}.
  This is similar to the no-change condition represented by
 Equation (15) of  \cite{FangSaad07}, which stipulates that 
  $(G_j - G_{j-m}) q = 0$ for all $q$ orthogonal to the span of the
  subspace $\Span \{ {\cal F}_j \}$ mentioned above, provided we define
 $ G_{j-m}= 0$. 

More links can be identified when setting $\beta = 0$ in Anderson acceleration.
Without loss of generality  and in an effort  to simplify notation we also \textcolor{red}{YX: do we have to assume this?}\textcolor{blue}{assume that $j_m = 1$ each time.}
 According to
 (\ref{eq:AA}--\ref{eq:thetaj}), the $j$-th iterate becomes simply
 $x_{j+1} = x_j - \FF_j \theta_j $ where
 $\theta_j$ is a vector that minimizes $\| f_j - \FF_j \theta \|$.
 For nlTGCR, we have $x_{j+1} = x_j + P_j y_j $
 where $y_j $ minimizes $ \| f(x_j) + V_j y \| $. So this  is identical with
 Equation \nref{eq:AA} when $\beta = 0$  in which  $P_j \equiv \XX_j$,
 and $\FF_j$ is replaced by $V_j$:
 
   \bigskip
 \begin{center}
 \begin{tabular}{c|c}
   AA         & nlTGCR  \\ \hline
   $\XX_j$    & $P_j$   \\
   $\FF_j$    & $V_j$ \\
   $\theta_j$ &  $- y_j$ \\
  \end{tabular}
  \end{center}

  \bigskip

  The most important relation for both cases is the multi-secant relation.
  For Anderson, we have
  \[ \FF_j = [f_1 - f_0, f_2 - f_1, \cdots, f_j - f_{j-1}] \quad
    \XX_j = [x_1 - x_0, x_2 - x_1, \cdots, x_j - x_{j-1}] \]
  and, with  $ G_{j-m} = 0 $,    the multi-secant matrix in \nref{eq:msec} becomes
  \eq{eq:AAb0}
    G_{j} = \XX_j  (\FF_j^T\FF_j)^{-1}\FF_j^T.
  \en 
  In the next proposition, we prove that 
  \begin{proposition}
  $G_{j}$ defined in \eqref{eq:AAb0} minimizes $ \| G \|_F$ for matrices $G$ that satisfy
  \[
    G \FF_j = \XX_j 
  \]
  \textcolor{red}{YX: the no-change condition $(G_j - G_{j-m}) q = 0$ for all $q$ orthogonal to the span of the
  subspace $\Span \{ {\cal F}_j \}$ equivalent to $G_j^T(G_j-G$?}
\textcolor{blue}{and the no-change condition
  \[
    G_j^T (G_j  - G) = 0.
  \]
  }
    \end{proposition}
  \begin{proof}
    Let $G$ a matrix as specfied above and set $\Delta = G_j - G$.
    Then
    \[ \| G \|_F^2 = \| G_j + \Delta \|^2 = \| G_j\|^2  + 2
      \underbrace{\Tr{G_j^T \Delta}}_{= 0}  + \|\Delta\|_F^2  \ge  \| G_j\|^2  . 
      \]
    \end{proof}

    Consider now nlTGCR. If we set $\FF_j \equiv V_j $ and $\XX_j = P_j$ in Anderson,
    the multisecant matrix $G_j$ in \nref{eq:AAb0} simplifies to \nref{eq:msecant1M} -
    which also minimizes $\|G \|_F$ under the secant conditopn
    $G V_j = P_j$ and the \textcolor{red}{YX: is the no-change condition \eqref{eq:msecant2} is equivalent to $G_j^T(G_j-G)$?} \textcolor{blue}{no-change condition $G_j^T (G_j - G) = 0$}.

    Therefore the two methods differ mainly in the way in which the sets
    $\FF_j / V_j$ ,  and $\XX_j / P_j $ are defined. Let us use the more general notation
    $V_j, P_j$ for the pair of subspaces. 

    In both cases, a vector $v_j$ is related to the corresponding $p_j$ by the fact that
    \eq{eq:ApproxNLT} v_j \approx J(x_j) p_j . \en
    In the case of nlTGCR this relation is explicitly enforced by
    a Frechet differentiation  (Line 10)-- before we perform an orthogonalization - which
    combines this vector with others -- without changing the span of the new $P_j$ (and also
    $V_j$). 

    In the case of AA, we have  $v_j = \Delta f_{j-1} = f_j - f_{j-1} $ and the relation exploited
    is that
    \eq{eq:ApproxAA}
    f_j \approx f_{j-1} + J(x_{j-1}) (x_j - x_{j-1}) \to
      \Delta f_{j-1} \approx J(x_{j-1}) \Delta  x_{j-1}
      \en

      
      However, relation \nref{eq:ApproxNLT} in nlTGMR is \emph{more accurate}- because we use an additional
      function evaluation to explicitly obtain  a more accurate approximation (ideally exact
      value)  for  $J(x_j) p_j$. In contrast when $x_j$ and $x_{j-1}$ are not close, then
      \nref{eq:ApproxAA} can be a very rough approximation. This is a key difference between the two
      methods. 
      \textcolor{red}{YX: Need experiments to verify this numerically.}
    

\textcolor{blue}{
      We also need to compare the two pairs of subspaces used: $P_j, V_j$ on the one hand
      and $\XX_j, \FF_j$ on the other.
      --- to be continued --- }
      
    
    
    
    
  
\iffalse  
 According to our earlier observation, $\XX_j$ is essentially the same as our $P_j$ - except for
 a scaling of the vectors. In addition, $\FF_j$ plays the role of our $V_j$ and
 what we call $y_j$ is the vector $\theta_j$ of AA. 
 If we had $\FF_j = V_j$ (up to scaling) the two methods would be identical.
 The only difference is the way in which the columns of $V_j$ are computed. It is important to note
 that 
\fi 






\subsection{Eigenvalue estimates as by-products}


We begin by reproducing the GCR algorithm for the linear case - in the situation when
$A$ is symmetric. In this case recall that the $\beta_{ij}$'s are all zero except
$\beta_{jj} $ which we now denote by $\beta_j$ (similar notation to CG)

We know that there is a strong relation between the Conjugate Gradient method and the
Lanczos vectors and this relation can provide eigenvalue estimates for the matrix $A$ in the
linear case -- see \cite[sec. 6.7.3]{Saad-book3}. It is also possible to derive a similar
result for the GCR algorithm. We wish to obtain a 3 term recurrence for building
an orthonormal basis of a Krylov subspace. Since the $A p_i$s are orthonormal it is natural to
consider these vectors.

As before we define  $v_j \equiv Ap_j$.
From Line~7 we get, upon multiplying through by $A$:
\eq{eq:Apj}
v_{j+1} = A r_{j+1} - \beta_j v_j
\en
But substituting the expresion of $r_{j+1}$ from Line~6 yields:
\eq{eq:Apj1}
v_{j+1} = A [r_j - \alpha_j v_j] - \beta_j v_j = = A r_j - \alpha_j A  v_j - \beta_j v_j .
\en
Next, from Line~7 used with $j$ instead of $j+1$ we have
$p_j = r_j - \beta_{j-1} p_{j-1}  \to
A r_j = v_j + \beta_{j-1} v_{j-1} $ and so we end up with:
\eq{eq:Apj2}
v_{j+1} = - \alpha_j A v_j + (1  - \beta_j)  v_j + \beta_{j-1} v_{j-1}
\en


  --------------------

  We rewrite the relation on the $v_i$s as
\[ 
  A v_j =  \frac{-1}{\alpha_j} v_{j+1}
  + \frac{1-\beta_j}{\alpha_j} v_{j}  + \frac{\beta_{j-1}}{\alpha_j} v_{j+1}   \]


This means that we have a tridiagonal representation of the matrix $A$ in the subspace
spanned by the $v_i$'s. This is identical with the Lanczos procedure.

--------------------

ALTERNATIVE PROJECTION METHODs. (1)
The above approach is not the only one if we want to estimate eigenvalues of $A$.
A second approach is to exploit the availabality of the bases $P$ and $AP$
and the fact that $AP$ is orthonormal.
We seek an approximate eigenpair
$\tilde \lambda, \tilde u$ where $\tilde  u  = P y$. Then writinf the Galerkin condition
\[
  (A - \tilde \lambda I) P y \perp \Span [A P]
\]
leads to 
\[
  (AP)^T (A - \tilde \lambda I) P y = 0
  \to [I - \tilde  \lambda P^T A P] y = 0
    \to [\frac{1}{\tilde  \lambda} I - P^T A P] y = 0 
\]
The advantage of the approaches discussed so far is that the matrices involved
are readily available and do not require any additional computations with
$A$. In the second case shown here we only need to compute inner products to get
$P^T A P$. 

ALTERNATIVE PROJECTION METHODs. (2)

We can also project only span(P) orthogonally to span(P)
Now we also seek an approximate eigenpair
$\tilde \lambda, \tilde u$ where $\tilde u = P y$ but the  Galerkin condition becomes
\[
  (A - \tilde \lambda I) P y \perp \Span [ P]
\]
which leads to a generalized eigenvalue problem 
\[
  (P)^T (A - \tilde \lambda I) P y = 0
  \to  P^T A P y =  \tilde \lambda  (P^T P ) y
\]
\fi 


